Edge Computing for IoT: Novel Insights from a Comparative Analysis of Access Control Models

IoT edge computing positions computing resources closer to the data sources to reduce the latency, relieve the bandwidth pressure on the cloud, and enhance data security. Nevertheless, data security in IoT edge computing still faces critical threats (e.g., data breaches). Access control is fundamental for mitigating these threats. However, IoT edge computing introduces notable challenges for achieving resource-conserving, low-latency, flexible, and scalable access control. To review recent access control measures, we novelly organize them according to different data lifecycles--data collection, storage, and usage--and, meanwhile, review blockchain technology in this novel organization. In this way, we provide novel insights and envisage several potential research directions. This survey can help readers find gaps systematically and prompt the development of access control techniques in IoT edge computing under the intricacy of innovations in access control.

==> Tex/Access_Control_Edge_Computing.tex <==
%\section{Access Control in Edge Computing}


\section{Access control in data collection}
\label{Sec::ACInDataCollection}

An abundance of raw data measured from IoT devices should be securely collected for subsequent processing and valuable insights. 
%The access control requirement is copied from Section III and pasted: \textit{
Access control should determine which IoT-generated raw data can be accessed by which services, meanwhile the access control should be flexible given the flexibility of end devices and services. For the processed raw data (i.e., intermediate data), access control should determine which intermediate data can be accessed by which edge service or cloud service.
In this section, we present the studies according to the typical model used as the base model to meet the access requirements, with the summary and lessons learned from these studies. 

\textit{GBAC as the base model:} To protect IoT-generated data from tampering and unauthorized access, group key management (GKM) is proposed \cite{grammatikis2019securing}. A device group key is shared with its current subscribers, and the device can encrypt its data by using a group key and only the legal subscribers can decrypt it. This ensures that authorized group users can access the data collected from IoT devices. However, the GKM only assigns a symmetric group key to each group and does not support members' independence in the same group. This means that keys need to be reassigned every time membership changes or state changes in a group. The flexibility in the IoT environment can induce frequent key redistribution and thus introduce large management and communication overhead. To conquer the challenges, Dammak et al \cite{dammak2020decentralized} propose a new decentralized lightweight group key management architecture for access control. It introduces a layered architecture, where a central key distribution center accounts for the management of the device group. 
Each device group has several user groups, and each user group corresponds to a sub-key distribution center (SKDC). By dispersing the key management tasks across multiple SKDCs, the system can better handle the complexity and overhead caused by changes in membership. When a user joins or leaves a group, only the SKDC where the user is located is adjusted.


\textit{TBAC as the base model: }Jiang et al. \cite{jiang2022trust} present a trust-based energy-efficient data collection for unmanned aerial vehicles (UAV). A UAV trajectory optimization algorithm recognizes the most data collection anchors, which guarantees the data collection trajectory is shortest and extends network life, meanwhile, a trust reasoning and evolution mechanism is used to identify the trusted sensor nodes and guarantee the quality of collected data. This method increases the network life by 48.9\%, and achieves 91\% accuracy in node trust degree identification while consuming only 8\% of network life.
%To enforce access control for mobile devices between edge nodes, Dang and Hoang \cite{dang2017data} build a region-based trust-aware model.
%It establishes trust between edge regions (each region connecting with various IoT devices), the mutually trusted regions can exchange and collect information about their IoT devices, such that, IoT devices can join or leave a region conveniently. 
%However, this work does not consider whether the received data is trustworthy (e.g., data may be tampered with). 

\textit{RAAC as the base model:} Atlam et al.\cite{atlam2021fuzzy} propose a dynamic and adaptive RAAC model. 
The risk assessment algorithm considers contextual information, resource sensitivity, action severity, and previous risk history. This model can adapt to the dynamics of IoT. When an access request is issued for data collection, the model can use the real-time characteristics of user requests to estimate the security risk and make an access decision. However, this solution is not evaluated.


% Praharaj et al. \cite{10061745}  propose an operational ReBAC model for smart IoT systems, referred to as ReBAC$_{\textit{IoT}}$, 
% a dynamic fine-grained model. When users request access to devices and information, ReBAC$_{\textit{IoT}}$ captures different user, session, device, operation, and environment attributes, and considers complex social relationships between subjects (users) and objects (resources) to make access control decisions.


\begin{table*}[]
\centering
\caption{Access control schemes in data collection}
\label{Table::ACCollection}
\begin{tabular}{|c|c|c|p{6cm}|p{5.5cm}|}
\hline
Ref & Base Model & Requirements & Performance & Key Improvements \\ \hline 
\cite{grammatikis2019securing, dammak2020decentralized}
   & GBAC  & \textbf{RC1}     &  High flexibility and scalability, Storage cost (Bytes), Computation cost (us), and Communication cost (us).  
   & Introducing a decentralized lightweight group key management scheme for flexible and scalable data collection.                            \\ \hline 
\cite{jiang2022trust}
   & TBAC  & \textbf{RC1}       &  Increasing the network life by 48.9\%, and achieving 91\% accuracy in node trust degree identification while consuming only 8\% of network life
   & Significantly improving the identification accuracy of node trust degree and greatly prolonging the network life.                            \\ \hline 
 \cite{atlam2021fuzzy} 
    & RAAC  & \textbf{RC1}      & -        
    & Attempting to provide the algorithm for calculating the risk of user requests to adapt the flexibility and scalability of IoT devices. \\ \hline
\cite{dougherty2021apecs, AADEC, liu2022secure}
    &  CapBAC    & \textbf{RC1} \& \textbf{RC2}    &  Average latency of user token verification is 4.8 ms. Supporting efficient and quick token revocation for IoT devices and edge servers.  & Providing a distributed access control framework for pervasive edge computing services.    \\ \hline

     \cite{alrawais2017attribute}
    & CP-ABE   &  \textbf{RC2}       &    The time overhead involves the key generation, encryption, and decryption. It is proportional to the number of attributes.                               & Providing a protocol for encrypted key exchange based on CP-ABE to establish secure communication between edge nodes and the cloud.                             \\ \hline  \cite{zhang2022achieving}
    & CP-ABE  &  \textbf{RC2}  & The encryption time is increased slightly because of the bilateral fuzzy matching. However, the decryption and communication overheads are decreased significantly due to the outsourced matching workload to edges nodes.
    & Achieving data sharing with bilateral fuzzy matching in a secure cloud-edge communication environment.                               \\ \hline 
\end{tabular}
\end{table*}

%Lots of research about CapBAC is conducted for securely and efficiently providing services for collected data by edge servers. 
\textit{CapBAC as the base model:} An advanced access control framework (APECS) for pervasive edge computing is proposed \cite{dougherty2021apecs}, where the legitimated end devices/edge servers can lightly obtain services permission of available edge servers, i.e., the access control for collecting data from end to edge and edge to edge is supported simultaneously. APECS framework depends on the CapBAC, where the authorized token for users by service providers is a tuple, including the unique identifier of the service provider, a list of service identifiers, a certificate of the user, a list of authorization levels, and the token's expiry time. The authentication and authorization tasks are directly delegated to semi-trusted edge servers, rather than centralized cloud servers, such that network communication beyond the edge is avoided. Moreover, APECS supports efficient and quick token revocation for users and edge servers. 
However, the authentication token contains the user's identity, so privacy leakage could happen once the user's identity is parsed by servers. An anonymous and auditable distributed access control framework for edge computing (AADEC) is proposed \cite{AADEC} for overcoming the deficiency. In AADEC, the user identity information is hidden, which raises the bar for attackers sniffing user privacy.
Nevertheless, because of the data confidentiality, it is likely to induce fake data spreading issues. AADEC allows a trusted third party to achieve malicious data auditing or tracing, which further mitigates the threat in edge computing. Moreover, Liu et al. \cite{liu2022secure} improve the efficiency of access control in APECS by achieving batch service authorization.

%The aforementioned studies do not consider the data collection from edge nodes to the cloud. 
%is also included in edge computing.
%The access control requirement is copied from Section III and pasted: \textit{
%Access control should determine which data can be accessed by which cloud service.
%(\textbf{RC2}).}

\textit{CP-ABE as the base model:} 
% Implementing CP-ABE can achieve access control meanwhile keeping received data reliable. 
To guarantee the confidentiality and verifiability of transmitted encrypted data between edge nodes and the cloud,
%However, the key security is another concern.  
%To guarantee the security of the key, 
ARWA et al. \cite{alrawais2017attribute} design an encrypted key exchange protocol based on CP-ABE and digital signature. In particular, the edge node's shared key can only be obtained by the cloud or other edge node(s) with a set of legal attributes. The experimental results show that, in terms of the CP-ABE mechanism, the key generation time, the encryption time, and the decryption time are increased linearly with the number of attributes.
%prevents adversaries from accessing unauthorized keys among a group of edge nodes and cloud.   
% To provide reliable query results for some high-security applications (e.g., life-critical applications), Ke et al. \cite{gu2019secure} propose a secure data query framework. To implement access control in this framework, they leverage the asymmetric encryption algorithm to encrypt the transferred data, and the corresponding key can decrypt the data. 
However, the attributes in this protocol are defined centrally, limiting access control's flexibility.
To implement more flexible access control, Zhang et al. \cite{zhang2022achieving} propose a scheme FADS, where edge nodes and cloud can specify access policies respectively and fuzzy matching is allowed. 
The transmitted data can be decrypted if and only if the receivers' attributes successfully match the access policies defined by two sides (sender and receiver). This matching is fuzzy, that is, receiver attributes can satisfy access policy without a rigid access structure. This way can hide the accurate user attributes, and enhance privacy protection. 

%\noindent\textbf{Summary and Lessons Learned.}
\subsection{Summary and Lessons Learned}
\label{Sec::SALInDataCollection}

In this section, we have discussed the studies to satisfy \textbf{RC1 \& RC2}.
The approaches are summarized in Table \ref{Table::ACCollection}, and the learned lessons are as follows:

\begin{itemize}
    \item 
%As shown in Table \ref{Table::ACCollection}, we summarize the access control schemes in data collection from the following aspects: model, decentralization, condition, scalability, privacy, efficiency, and scenario. 
We can observe that these studies leverage various components to achieve access control, which facilitates data collection within the dynamic environment of edge computing. Some focus on developing algorithms to evaluate access control components, such as group, trust, and risk. 
%Relationships can be equipped to personalize data collection.
Others, addressing the challenges of resource-constrained IoT devices, incorporate different elements to create valid tokens in CapBAC. The high-performance implementation of CapBAC enables the effective use of edge services for processing IoT raw data.
%CP-ABE is researched for realizing secure and efficient data collection among edges and cloud, where data likely travels across different security domains.
However, privacy concerns, particularly regarding the sensitive elements in tokens, must be also addressed \cite{AADEC}.
Furthermore, when combined with data cryptography, these access control schemes can ensure secure and flexible data collection for smart IoT devices \cite{dammak2020decentralized}. 

\item 
Although components such as group, trust, risk, raw context, capability, and cryptography facilitate adaptive data collection in the dynamic environment of edge computing, their integration has not been thoroughly explored. 
%For example, a decentralized evaluation scheme for group, trust, and risk would be expected while data privacy is considered.
%In a high-dynamic environment, edge servers may provide new services or remove old services with developing businesses. 
% For example, some IoT devices would fuse data with other source data to get specific services. 
% We expect a high-performance CapBAC scheme, whose tokens support flexible and efficient capability registration, delegation, and revocation, and support federated operations to allow different data sources to obtain services collaboratively, and support finding optimal service location according to extra information (e.g., network topology from software-defined network \cite{goransson2016software}, group, and trust).
For instance, some IoT devices may integrate data from various sources to deliver specific services. A high-performance CapBAC scheme is desirable, which would support flexible and efficient token management—enabling capability registration, delegation, and revocation. It should also allow for federated operations, enabling collaborative service access across different data sources, and optimize service location using additional information, such as network topology from software-defined networks \cite{goransson2016software}, group dynamics, and trust levels.

\end{itemize}



% \begin{table*}[]
% \centering
% \caption{Comparison among access control schemes in edge computing from data collection}
% \label{Table::ACCollection}
% \begin{tabular}{|p{0.4cm}<{\centering}|p{1cm}<{\centering}|c|c|c|c|p{6.7cm}|p{6.7cm}|}
% \hline
% Ref & Model(s) & Decentralization & Base model & {\color{red}Scalability} %xt要去掉 
% & {\color{red} Privacy} % xt要去掉 
% & \multicolumn{1}{c|} {Performance} & \multicolumn{1}{c|}{Scenario} \\ \hline 
% \cite{dammak2020decentralized}
%    & DLGKM-AC                & \checked              & GBAC     & \checked           & \checked        & High scalability, Single member control, Storage cost 
%  (Bytes), Computation cost (us), Communication cost (us)                            & Introducing a decentralized lightweight group key management scheme for flexible and scalable data collection with dynamic edge nodes and IoT devices                            \\ \hline 
% % \cite{jiang2022trust}    & TBAC                & \checked              &  Trust    & -           &     -   &            -              & Introducing a trust management scheme for flexible and scalable data collection with unmanned vehicles as edge nodes.                             \\ \hline 
% \cite{CAABAC}
%    & CAABAC    & -             & CP-ABE\&CAAC   & \checked           & \checked        & Basic context, Storage cost (($\left|att\right|$+2)$\left|\mathbb{G}_{1}\right|$), Communication cost (bytes size), Computation cost (673.4ms in edge nodes, 0.1ms in IoT devices)                                  & Providing a contextual cryptography-based scheme for flexible data collection of smart IoT devices                                 \\ \hline 
%    \cite{atlam2021fuzzy} 
%     & Fuzzy logic RAAC               & -             & RAAC      & \checked            & -       & -                                 & Focusing on the algorithm for calculating the risk of user request to adapt the flexibility and scalability of IoT.                              \\ \hline \cite{10061745}
%     & ReBAC$_{IoT}$              & -              & ReBAC & \checked            & -       & With having multiple users and devices, the time cost is about several hundreds of ms.                                 & Realizing policy individualization according to users' social relationship and attributes                             \\ \hline \cite{dougherty2021apecs, AADEC, liu2022secure}
%     &   APECS, AADEC, SE-DAC         & \checked             & CapBAC         & -           & \checked       & \checked                                  & Focusing on solving the problem of distributed service access control in the edge computing environment                               \\ \hline 
%     % \cite{AADEC} & CapBAC             & -             & Capability         & -           & \checked        & \checked                                 & Achieving anonymous and auditable distributed access control in edge computing services                              \\ \hline \cite{liu2022secure}
%     % & CapBAC             & \checked               & Capability & \checked           & -       & \checked                                 &                                 \\ \hline 
%     \cite{dang2017data}
%     & TBAC             & -             & Trust        & -           & -       & \checked                                  & Focusing on data security and performance of fog nodes and their data as they move frequently in their environment                               \\ \hline \cite{alrawais2017attribute}
%     & CP-ABE             & -             & -         & \checked            & \checked        & \checked                                  & Providing a protocol for encrypted key exchange based on CP-ABE to establish secure communication between fog nodes and cloud                             \\ \hline \cite{gu2019secure}
%     & -                  & \checked  & -         & \checked            & -       & \checked                                  & Building a secure data query framework to achieve safe and reliable query operations on data in distributed storage                               \\ \hline \cite{zhang2022achieving}
%     & CP-ABE                  & -             & -         & \checked            & \checked        & \checked                                  & Achieving data sharing with fuzzy matching in a secure cloud-edge communication environment                               \\ \hline 
% \end{tabular}
%  \begin{tablenotes}
%      \item[1] $\left|\mathbb{G}_{1}\right|$: the size of a cyclic additive group of prime order q, $\left|att\right|$: the size of attributes number.
%    \end{tablenotes}
% \end{table*}

\section{Access control in data storage}
\label{Sec: ACInDataStorage}



As learned from typical access control models, ABE-based access control is popular data cryptography solutions for secure data storage in edge computing. The stored raw data should be protected by access control policies specified by data owners or administrators. The stored computation results may be cooperated among edge nodes/cloud, where different edge/cloud services should access different computation results.
This section introduces the corresponding recent studies. 

\subsection{ABE-based access control}
\label{Sec::Abe_based_AC}


We recommend the surveys \cite{ABESurvey, oberko2022survey} for readers to learn more about ABE.
We present the most recent studies, which include general ABE-based solutions, generalizing the common problems in edge computing, and domain-specific ones, which design ABE for edge computing of some domains. We first introduce the general ABE-based solutions.

   
% To encrypt users' data, APECS \cite{dougherty2021apecs} framework depends on multi-authority KP-ABE for achieving federated authority among semi-trusted edge servers. APECS accomplishes efficient asynchronous access control, where edge servers are allowed to be offline intermittently. 
% APECS does not concern the searchable applications, and cannot conduct fine-grained access control on ciphertext. Multi-keyword attribute-based searchable encryption (EMK-ABSE) \cite{liu2022emk} combines the ABE and searchable encryption, which simultaneously achieves data searchability and fine-grained access control on the ciphertext. EMK-ABSE stores encrypted data on cloud servers and uploads the corresponding encrypted index on the nearest edge nodes to achieve multi-keyword search and assisted decryption. In addition, EMK-ABSE utilizes the online/offline mechanism to optimize data encryption performance.



The linear relationship between the ciphertext/secret key sizes and the number of attributes impedes the development of ABE-based solutions. 
To address this issue, Sarma et al. \cite{sarma2022macfi} propose a multi-authority CP-ABE scheme MACFI, which reduces the data size and outsources expensive decryption computation to edge nodes. 
MACFI achieves that the size of the secret key is kept irrespective of the number of attributes and that the ciphertext size is agnostic for the number of attributes and has a linear relationship with the number of authorities. 
MACFI further increases the efficiency of CP-ABE-based access control for edge computing in IoT. Moreover, each attribute authority in MACFI verifies a user, and allocates attributes based on the user's role (RBAC).
Xu et al. \cite{xu2020match} propose a new matchmaking attribute-based encryption (MABE) for enhancing the performance of KP-ABE. On the one hand, MABE uses collision-resistant hash functions to generate the ciphertexts, which decreases the encryption time for IoT devices.
On the other hand, like outsourcing ciphertext decryption to edge nodes, MABE also outsources heavy ciphertext identification to edge nodes, but edge nodes can leverage the access structures from data receivers to filter useless data in the ciphertext. As such, the decryption time is decreased largely. 
As shown in the experiments, this way not only decreases the computation overhead for IoT devices garnering useful data but also saves the cost of bandwidth. 
% Xiong et al. \cite{9751084} propose a lightweight and verifiable multi-authority CP-ABE access control scheme, which makes ciphertext size constant and mitigates the computational cost by outsourcing decryption tasks for resource-limited IoT devices. Moreover, this work implements attribute revocation.


%The research efforts reduce the computation burden for resource-constrained IoT devices by controlling the ciphertext size. 
Changing the mathematics in cryptography is another way to cut down the computation burden. 
To consume much fewer resources, Rui et al. \cite{cheng2021efficient} propose a novel CP-ABE scheme based on elliptic curve cryptography. As a result, the expensive bilinear pairing operation in native CP-ABE is replaced with simple scalar multiplication. In addition, this study considers the time and location attributes for encryption and also outsources expensive computational tasks to edge servers. As shown by the experiments, the encryption of time and location attributes consumes a few scalar multiplication operations, and the decryption time has no obvious linear relationship with the number of attributes because the resource-limited IoT devices only calculate the scalar multiplication operation one time. 

The aforementioned studies commonly improve ABE-based access control efficiency by offloading the decryption computation burden to edge nodes.
To further improve the efficiency, Xu et al. \cite{xu2021server} reduce the cost of data decryption simultaneously by outsourcing the workloads from these aspects: data source identification, revocable storage, and decryption mechanism.



 
%Although the aforementioned studies leverage ABE for securing edge computing, they do not mainly focus on contextual access control. 
IoT gateway can sense the context information with IoT devices or vicinity users, e.g., location, time, and sensitivity. The context information often changes continuously and frequently, making the static and traditional security solutions inefficient. For example, Rui et al. \cite{cheng2021efficient} simply combine contextual attributes (time and location) with their CP-ABE solution. Arfaoui et al. \cite{CAABAC} propose a context-aware attribute-based access control (CAABAC) approach for providing data consumers with secure and adaptive remote control of smart IoT. CAABAC incorporates the CP-ABE with contextual information to achieve adaptive contextual data collection for data consumers, where contextual tokens are integrated into the CP-ABE's access structure. 
When data consumers decrypt the collected data, they are required an attribute set and context information to collectively satisfy the access structure. In this solution, IoT gateways act as edge nodes, which store the encrypted data. The experiments show that small computation cost is consumed on IoT devices.
However, the most existing CP-ABE solutions force data users to manually provide the contextual information for encrypting or decrypting data. This way indicates that malicious data users can conjecture which attributes are incorrect, such that it is possible to raise unauthorized access to information.
Ghosh et al. \cite{ghosh2021case} propose a context-aware attribute learning scheme CASE for tackling the issues. Depending on the edge intelligence, CASE can learn users' contextual attributes and generate attributes automatically, which could decrease manual operations and thus enhance the system's security. Meanwhile, it reduces the size of post-encryption data based on learned attributes, which increases the scalability of access control as discussed in the experiments. 
% Although the above efforts facilitate data security in edge computing by ABE-based access control, they do not consider the user's trust degree. 
Because a trust degree has regional characteristics in edge computing,
Zheng et al. \cite{zheng2022adaptive} propose an access control scheme based on CP-ABE, which combines users' trust degree.
The scheme leverages the classification and recommendation algorithms for adaptively determining users' trust degree in different regions. 
Therein, the trust degree is divided into three dimensions: the basic trust degree, the behavior trust degree, and the recommendation trust degree. The number of attributes in the scheme is constant, which decreases the computational overhead.
% Moreover, this work adopts the cryptographic auditing technique to support data integrity checking before the user obtains data while protecting privacy. Specially, the 
% To further facilitate data sharing and access, TODA strategy \cite{xia2019secure} is presented and designed.
% This strategy focuses on flexible data access, where unknown users could be evaluated by reputation centers for determining trust levels when data owners are unavailable. TODA is tailored for the RoSES model which realizes robust and secure edge storage without privacy leakage when failed data is recovered. The experiment shows that the time of decrypting data is under 1ms.

\begin{table*}[]
\centering
\caption{General access control schemes in data storage}
\label{Table::ACStorage}
\begin{tabular}{|c|c|c|p{6cm}|p{5.5cm}|}
\hline
Ref & Base Model & Requirements & Performance & Key Improvements \\ \hline 
\cite{sarma2022macfi}
   & CP-ABE  & \textbf{RS1}\&\textbf{RS2}     & Computation cost: Key generation ($2N_{A_{u}}$+$\left|\mathbb{A}\right|$)$T_{G}$, Encryption ($3N_{A_{u}}$+2(n-$\left|\mathbb{P}\right|$))$T_{G}$ + $T_{G_{T}}$, Decryption ($\left|\mathbb{A}\right|$-$\left|\mathbb{P}\right|$)$T_{G}$+$N_{A_{p}}$$T_{G_{T}}$+$3N_{A_{p}}$$T_{p}$. Ciphertext size: $3N_{A_{p}}$$\left|G\right|$+2$\left|G_{T}\right|$, Key size: $\left|Z_{p}\right|$.
   & The size of the secret key is kept irrespective of the number of attributes and the ciphertext size is agnostic for the number of
attributes and has a linear relationship with the number of
authorities                           \\ \hline 
\cite{xu2020match}
   & KP-ABE  & \textbf{RS1}\&\textbf{RS2}       &  Computational complexity: Encryption $\mathcal{O}$($\mathcal{S}$+$\mathcal{R}$), Decryption $\mathcal{O}$($\mathbb{R}$). Space Complexity: Encryption key $\mathcal{O}$($\mathcal{S}$), Decryption key $\mathcal{O}$($\mathbb{R}$).
   & Filtering useless data in the ciphertext for IoT devices (as data receivers) according to more constraints of data producers and consumers.                            \\ \hline 
 \cite{cheng2021efficient}
    & CP-ABE  & \textbf{RS1}\&\textbf{RS2}       & 
    Computation cost: Encryption (4$N_{r}$+1)G, Decryption [at edge] ($D_{a}$+1)G, Decryption [at end device] G. Ciphertext size (3$N_{r}$+1)$|G^{'}|$, Public key size (2n+2)$|G^{'}|$, Private key size $|\mathbb{P}|$ $|G^{'}|$.
    & Cutting down the computation burden for resource-limited IoT devices by changing the mathematics in cryptography. \\ \hline
 \cite{xu2021server}
    &  CP-ABE    & \textbf{RS1}\&\textbf{RS2}   &  Computational complexity: Key generation $\mathcal{O}$(1), Encryption $\mathcal{O}$($\mathcal{S}$+$\mathbb{R}$), Decryption $\mathcal{O}$($1$). & Reducing the computation burden for resource-limited IoT devices from multiple aspects.   \\ \hline
    
    \cite{CAABAC}
    & CP-ABE  &   \textbf{RS1}\&\textbf{RS2}   &     Storage overhead: $(\left|\mathbb{A}\right|+2)\left|{G}_{1}\right|$
    ,
    Communication overhead: 359 bytes (IoT gateway), 16 bytes (Smart thing), Computation cost: 673.4ms (IoT gateway), 0.1 ms (Smart thing)
    & Introducing context into CP-ABE and providing dynamic access control.                               \\ \hline 
     \cite{ghosh2021case} 
    & CP-ABE   &  \textbf{RS1}\&\textbf{RS2}      &           The study mainly evaluates average network delay, average energy consumption, and average packet loss. In each metric, CASE has significant improvement by about 33\%.                      & Introducing edge intelligence to avoid manually providing
context information and sensitive data inference.                             \\ \hline 
    \cite{zheng2022adaptive} 
    & CP-ABE   &  \textbf{RS1}\&\textbf{RS2}      &           Due to the three-levels trust degree, the number attributes of is constant.                     &  Depending on AI to determine the trust degree of users in different regions adaptively, and combining CP\_ABE with the trust degree.                             \\ \hline 
\end{tabular}
 \begin{tablenotes}
     \item[1] Table \ref{Table::Notations} provides descriptions for various notations.
   \end{tablenotes}
\end{table*}

\begin{table*}[]
\centering
\caption{Notations}
\label{Table::Notations}
\begin{tabular}{|c|l|}
\hline
Notation & Description \\ 
\hline
AAs & attribute authorities \\
\hline
n & Total number of attributes in the system \\
\hline
$\left|\mathbb{P}\right|$ & Number of attributes in access policy $\mathbb{P}$\\
\hline
$\left|\mathbb{A}\right|$ & Number of attributes in user’s attribute set $\mathbb{A}$\\
\hline
$N_{A_{p}}$ &  Number of AAs whose attributes are used in policy $\left|\mathbb{P}\right|$ \\
\hline
$N_{A_{u}}$ &  Number of AAs whose attributes are used in user's attribute set $\left|\mathbb{A}\right|$ \\
\hline
$T_{G}$ & Time to execute an exponentiation operation in an element of source groups $G_{1}$ and $G_{2}$ \\
\hline
$T_{G_{T}}$ & Time to execute an exponentiation operation in an element of target group $G_{T}$ \\
\hline
$T_{p}$ & Time to execute one pairing operation \\
\hline
$\left|Z_{p}\right|$ & Size of an element of $Z_{p}$ \\
\hline
$\left|G\right|$ & Size of an element of source group $G_{1}$ and $G_{2}$ \\
\hline
$\left|G_{T}\right|$ & Size of an element of target group $G_{T}$\\
\hline
$\mathcal{S}$, $\mathcal{R}$ & Attribute sets of a sender and a receiver \\
\hline
$\mathbb{S}$, $\mathbb{R}$ & Policies associated with a sender and a receiver \\
\hline
$N_{r}$ & Number of rules in $\left|\mathbb{P}\right|$ \\
\hline
Da &  Minimum number of attributes satisfying the access policy \\
\hline
$|G^{'}|$ & 160 bits considered as a unit of measurement \\
\hline
\end{tabular}
\end{table*}

The aforementioned studies provide general considerations for enhancing the performance of ABE in edge computing. Apart from these general considerations, we should have some access control schemes for specific domains. We next simply present some studies in transportation and healthcare domains. 
% In mobile edge computing (e.g., mobile phones and cars), ABE solutions are also investigated. 
% Zhang et al. \cite{FDO-ABE} proposes a fully decentralized outsourced ABE scheme FDO-ABE, which provides access control for mobile edge computing with distributed microdata storage. FDO-ABE relies on a non-interactive multi-authority CP-ABE scheme, which not only supports the multi-attribute authorities in generating the multi-attribute-based private keys for the user but also provides the independent and isolated ciphertext storage for the distributed cloudlets nodes.

In the realm of transportation, 
edge computing is vital for conducting data access with low latency, and ABE-based access control is researched correspondingly. For example, OpenVDAP \cite{OpenVDAP}, an open full-stack edge computing-based platform, is dedicated to achieving low-latency data analytics for connected and autonomous vehicles (CAVs). Vehicle sensing data include historical data and real-time data, and different data sources have different access patterns. AC4AV \cite{AC4AV} first defines the data access control problem in CAVs. AC4AV can support various access control models (including ABE) by allowing users to dynamically adjust and customize access control models. AC4AV is implemented based on the OpenVDAP platform.  
To address the security and privacy issues in car-hailing systems, Sun et al. \cite{sun2022practical} propose a fine-grained puncturable matchmaking encryption (FP-ME) based on MABE and puncturable encryption. In FP-ME, not only the fine-grained access control between passengers and drivers about orders can be achieved, but also, the privacy and authenticity of passengers' orders are protected and the timeliness of passengers' ciphertext orders is guaranteed.
To achieve secure data sharing in intelligent autonomous vehicle platoons, Sun et al. \cite{sun2022secure} 
initially propose a privacy-preserving data share mechanism with flexible cross-domain authorization (FDSM-FC). In FDSM-FC, the privacy-preserving matchmaking encryption technology is combined with the cross-domain transformation primitive. In this way, it exploits the dual merits of those technologies and achieves data authenticity and authorization simultaneously.
In addition, Bao et al. \cite{9830119} present an EA-PH-ABE-DS scheme in the Internet of Vehicles (IoV) scenario where data services are expected to be more flexible and diversified. EA-PH-ABE-DS efficiently supports the update of ciphertext and user secret key in IoV and leverages edge computing to reduce computation overhead further.

In the health care domain, Zhang et al. \cite{zhang2021lightweight} design a lightweight and fine-grained access control for electronic medical record sharing systems. Therein, symmetric encryption is used to encrypt medical records by data owners and ABE is used to protect symmetric key.  
Hassan Nasiraee and Maede Ashouri-Talouki \cite{nasiraee2021privacy} propose a new privacy-preserving distributed data access control (PDAC). In PDAC, a new user anonymity approach, a novel policy-hiding mechanism, and an independent authority system are simultaneously considered for improving privacy preservation.
The anonymity approach and policy hiding can prevent untrusted authorities from colluding, and the authority system adds/removes an authority without reinitializing other authorities.  


%\subsection{PRE-based access control}

% Canetti et al.\cite{ateniese2006improved} present a unidirectional PRE scheme based on bilinear pairings. The scheme is only secure against chosen-plaintext attacks, however, applications often require security against chosen-ciphertext attacks (CCA). To address this gap, Canetti and Hohenberger \cite{canetti2007chosen} present a construction of a CCA-secure bidirectional PRE scheme based on bilinear pairings.


% Although data owners in PRE can re-encrypt data through the proxy without disclosing the key or plaintext, the proxy can easily identify the participants (data owner and data consumer) involved in the re-encryption process, which poses a major security concern. To address this issue, Ateniese et al. \cite{ateniese2009key} propose the key-private PRE, where the re-encryption key is generated by blinding the public key, and the proxy cannot identify the generator of the blinded key. 
% Dan Boneh et al.\cite{boneh2001identity} propose the ID-based PRE which does not need public-key infrastructure and a secure database to store key pairs. However, the geographically dispersed nature of edge nodes makes them vulnerable to side-channel attacks that can cause key leakage. 

% To effectively resist continuous key leakage caused by such attacks, Wang\cite{wang2018leakage} proposes a leakage-resilient ID-based PRE.


% Despite these improvements, PRE may not be adequate to handle scenarios that require fine-grained delegation. To address this limitation, Weng et al. \cite{weng2009conditional} propose the conditional proxy re-encryption (C-PRE), where only ciphertext satisfying a specific condition set by the data owner can be re-encrypted by the proxy and decrypted by the data consumer. Zeng et al. \cite{zeng2018new} propose an improved C-PRE approach, which enables the proxy to transform only ciphertext from a specified sender. 

 
% In addition, the re-encryption process places a significant computational burden on the proxy, leading to processing latency issues. To overcome this challenge, Khashan \cite{khashan2020hybrid} proposes a hybrid PRE scheme by combining lightweight symmetric and asymmetric encryption algorithms, which greatly saves on the computation cost of encryption, re-encryption, and decryption processes. Similarly, Hassan et al. \cite{hassan2021research} propose a certificate-based incremental PRE scheme to solve the delay problem caused by the application of PRE to electronic medical data sharing on edge computing.


\subsection{Summary and Lessons Learned}
In this section, we have discussed the studies to satisfy \textbf{RS1}\&\textbf{RS2}. Some approaches are summarized in Table \ref{Table::ACStorage} for the discussion, and
learned lessons are as follows:

%To present the discussions and envisage future directions about access control in data storage, we select several research works of ABE (shown in Table \ref{Table: ACofECDataStorage}).
%Due to the architecture of edge computing, they generally work on MA-ABE. 
%We summarize the access control solutions from the following aspects: offloading, data size reduction, AI assistance, condition, and scenario. 
%From these aspects, we discuss the lessons for achieving the high-performance data cryptography for access control. 

\begin{itemize}
    \item 
\textit{Rational use of computing power:} In these research studies, resource-constrained IoT devices leverage the computing powers from third parties (e.g., edge nodes and cloud) to offload the computing load from cryptography algorithms.
Most works simply and rigidly outsource the whole computing tasks by neighbor edge servers. 
The outsourcing model indicates that IoT devices need neighbors with relatively ample resources. 
However, the neighbors may have different computing resources. 
For example, general CPU-based edge servers can achieve outsourced computing tasks. Also, ASIC is designed for accelerating data encryption/decryption \cite{gaj2009fpga}. Moreover, the network from IoT devices to neighbors changes randomly. For example, edge servers intermittently offline, and large traffic induces network congestion \cite{EssentialsofEC}.
It is advisable to have more flexible task-offloading strategies for cryptography algorithms, which could improve the availability of computing power. Such that, resource access can be controlled more efficiently in pervasive edge computing by more rational use of computing power.


% \begin{table*}[]
% \centering
% \caption{General access control schemes in data storage}
% \label{Table::ACStorage}
% \begin{tabular}{|c|c|c|p{6cm}|p{5.5cm}|}
% \hline
% Ref & Base Model & Requirements & Performance & Key Improvements \\ \hline 
% \cite{sarma2022macfi}
%    & CP-ABE  & \textbf{RS1}\&\textbf{RS2}     & Computation cost: Key generation ($2N_{A_{u}}$+$\left|\mathbb{A}\right|$)$T_{G}$, Encryption ($3N_{A_{u}}$+2(n-$\left|\mathbb{P}\right|$))$T_{G}$ + $T_{G_{T}}$, Decryption ($\left|\mathbb{A}\right|$-$\left|\mathbb{P}\right|$)$T_{G}$+$N_{A_{p}}$$T_{G_{T}}$+$3N_{A_{p}}$$T_{p}$. Ciphertext size: $3N_{A_{p}}$$\left|G\right|$+2$\left|G_{T}\right|$, Key size: $\left|Z_{p}\right|$.
%    & The size of the secret key is kept irrespective of the number of attributes and the ciphertext size is agnostic for the number of
% attributes and has a linear relationship with the number of
% authorities                           \\ \hline 
% \cite{xu2020match}
%    & KP-ABE  & \textbf{RS1}\&\textbf{RS2}       &  Computational complexity: Encryption $\mathcal{O}$($\mathcal{S}$+$\mathcal{R}$), Decryption $\mathcal{O}$($\mathbb{R}$). Space Complexity: Encryption key $\mathcal{O}$($\mathcal{S}$), Decryption key $\mathcal{O}$($\mathbb{R}$).
%    & Filtering useless data in the ciphertext for IoT devices (as data receivers) according to more constraints of data producers and consumers.                            \\ \hline 
%  \cite{cheng2021efficient}
%     & CP-ABE  & \textbf{RS1}\&\textbf{RS2}       & 
%     Computation cost: Encryption (4$N_{r}$+1)G, Decryption [at edge] ($D_{a}$+1)G, Decryption [at end device] G. Ciphertext size (3$N_{r}$+1)$|G^{'}|$, Public key size (2n+2)$|G^{'}|$, Private key size $|\mathbb{P}|$ $|G^{'}|$.
%     & Cutting down the computation burden for resource-limited IoT devices by changing the mathematics in cryptography. \\ \hline
%  \cite{xu2021server}
%     &  CP-ABE    & \textbf{RS1}\&\textbf{RS2}   &  Computational complexity: Key generation $\mathcal{O}$(1), Encryption $\mathcal{O}$($\mathcal{S}$+$\mathbb{R}$), Decryption $\mathcal{O}$($1$). & Reducing the computation burden for resource-limited IoT devices from multiple aspects.   \\ \hline
    
%     \cite{CAABAC}
%     & CP-ABE  &   \textbf{RS1}\&\textbf{RS2}   &     Storage overhead: $(\left|\mathbb{A}\right|+2)\left|{G}_{1}\right|$
%     ,
%     Communication overhead: 359 bytes (IoT gateway), 16 bytes (Smart thing), Computation cost: 673.4ms (IoT gateway), 0.1 ms (Smart thing)
%     & Introducing context into CP-ABE and providing dynamic access control.                               \\ \hline 
%      \cite{ghosh2021case} 
%     & CP-ABE   &  \textbf{RS1}\&\textbf{RS2}      &           The study mainly evaluates average network delay, average energy consumption, and average packet loss. In each metric, CASE has significant improvement by about 33\%.                      & Introducing edge intelligence to avoid manually providing
% context information and sensitive data inference.                             \\ \hline 
%     \cite{zheng2022adaptive} 
%     & CP-ABE   &  \textbf{RS1}\&\textbf{RS2}      &           Due to the three-levels trust degree, the number attributes of is constant.                     &  Depending on AI to determine the trust degree of users in different regions adaptively, and combining CP\_ABE with the trust degree.                             \\ \hline 
% \end{tabular}
%  \begin{tablenotes}
%      \item[1] Table \ref{Table::Notations} provides descriptions for various notations.
%    \end{tablenotes}
% \end{table*}

% \begin{table*}[]
% \centering
% \caption{Notations}
% \label{Table::Notations}
% \begin{tabular}{|c|l|}
% \hline
% Notation & Description \\ 
% \hline
% AAs & attribute authorities \\
% \hline
% n & Total number of attributes in the system \\
% \hline
% $\left|\mathbb{P}\right|$ & Number of attributes in access policy $\mathbb{P}$\\
% \hline
% $\left|\mathbb{A}\right|$ & Number of attributes in user’s attribute set $\mathbb{A}$\\
% \hline
% $N_{A_{p}}$ &  Number of AAs whose attributes are used in policy $\left|\mathbb{P}\right|$ \\
% \hline
% $N_{A_{u}}$ &  Number of AAs whose attributes are used in user's attribute set $\left|\mathbb{A}\right|$ \\
% \hline
% $T_{G}$ & Time to execute an exponentiation operation in an element of source groups $G_{1}$ and $G_{2}$ \\
% \hline
% $T_{G_{T}}$ & Time to execute an exponentiation operation in an element of target group $G_{T}$ \\
% \hline
% $T_{p}$ & Time to execute one pairing operation \\
% \hline
% $\left|Z_{p}\right|$ & Size of an element of $Z_{p}$ \\
% \hline
% $\left|G\right|$ & Size of an element of source group $G_{1}$ and $G_{2}$ \\
% \hline
% $\left|G_{T}\right|$ & Size of an element of target group $G_{T}$\\
% \hline
% $\mathcal{S}$, $\mathcal{R}$ & Attribute sets of a sender and a receiver \\
% \hline
% $\mathbb{S}$, $\mathbb{R}$ & Policies associated with a sender and a receiver \\
% \hline
% $N_{r}$ & Number of rules in $\left|\mathbb{P}\right|$ \\
% \hline
% Da &  Minimum number of attributes satisfying the access policy \\
% \hline
% $|G^{'}|$ & 160 bits considered as a unit of measurement \\
% \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[]
% \centering
% \caption{Comparison among access control schemes in edge computing from data storage}
% \label{Table: ACofECDataStorage}
% \begin{tabular}{|l|c|c|c|c|p{7.2cm}|}
% \hline
% \multicolumn{1}{|c|}{Scheme} &  Offloading  & Data size reduction & AI assistance & Condition  & \multicolumn{1}{c|}{Scenario}                                                                                              \\ \hline
% \cite{dougherty2021apecs}                   & -                   & -           & -          & -                                            & IoT devices store data on intermittently offline semi-trust edge servers                                                   \\ \hline
% \cite{liu2022emk}                     & Encrypted index & -                   & -           & -            & Achieving efficient data searchability and fine-grained access control on the ciphertext by exploiting edge nodes          \\ \hline
%  \cite{sarma2022macfi}  & Decryption & key and ciphertext  & -           & -                                                                   & Focusing on reducing data size and computation pressure for resource-limited IoT devices                                   \\ \hline
% \cite{xu2020match} & Decryption  & ciphertext          & -           & -                                                                  & Focusing on filtering useless data in the ciphertext for IoT devices (as data receivers) according to more constraints of data producers and consumers                                  \\ \hline
% \cite{9751084}   & Decryption & ciphertext          & -           & -                                                              & Providing a lightweight and verifiable MA-CP-ABE for resource-limited IoT devices                                          \\ \hline
% \cite{cheng2021efficient}   & Decryption & ciphertext          & -           & context         & Cutting down the computation burden for resource-limited IoT devices by changing the mathematics in cryptography           \\ \hline
%  \cite{xu2021server}  & Decryption and other & -                   & -           & group    & Reducing the computation burden for resource-limited IoT devices from multiple aspects                                     \\ \hline
% \cite{zheng2022adaptive}   & - & -                   & \checked    & trust                                                                        & Adaptively determining the trust degree of users in different regions                                                      \\ \hline
% \cite{xia2019secure}  & -  & -                   & -           & trust      & Improving edge storage model to offer security-aware data robustness and adaptable data sharing among many uncertain users \\ \hline
% \cite{CAABAC}   & -      & -                   & -           & context  & Introducing context into CP-ABE and providing dynamic access control                                                       \\ \hline
% \cite{ghosh2021case}           & -     & ciphertext       & \checked & context      & Introducing edge intelligence to avoid manually providing context information and sensitive data inference                 \\ \hline
% \end{tabular}
% \vspace{-0.1cm}
% \end{table*}







\item
\textit{Reduction in computational power requirements:} Larger key size and ciphertext size need more computing resources regardless of the usage strategies of computing power. Some research studies focus on improving the performance of cryptography-based schemes by cutting down these sizes or making them constant. 
However, these solutions reduce the expressive capability of access policy, i.e., the system's ability to satisfy ample security requirements is declined.
We should consider a trade-off between policy expressiveness and data size. 
Besides, reducing the requirement for computing power appropriately is labor-intensive and expert. 
It could facilitate the development of cryptography-based access control if we make that trade-off easier for general engineers.


\item
\textit{Introduction of additional access control components:} In different application scenarios, various components for access control are utilized, including bilateral practitioners, trust, context information, etc.
For example, edge nodes and cloud are bilateral practitioners for determining which IoT devices can access stored data. In this way, access policy is considered with more components, as a result, more useless data can be previously filtered for IoT devices by more constraints. 
The trust of data users is a factor for dynamically determining whether encrypted data can be decrypted. 
Context evaluates whether the current time or location is satisfied for decrypting data. 
In edge computing, we cannot sometimes pre-know which components are suitable for which scenario. 
Automatically recognizing components for specific scenarios can facilitate data security in pervasive edge computing.    

\item 
\textit{Reduction in human power:} 
In the studies mentioned above, some use machine learning/deep learning to substitute human power for achieving functional components in access control systems.
In this way, the components, which conventionally need human power for maintenance, can be optimized enough, and as a result, the access control system can be more efficient.
For example, Ghosh et al. \cite{ghosh2021case} largely reduce the average network delay, energy consumption, and packet loss by integrating context-aware attributes learning scheme into CP-ABE.
In addition, data privacy in the system could be improved due to less human involvement. 
Machine learning-based access control should be researched further to introduce effective and efficient intelligent algorithms into access control schemes.
%, from the rational use of computing power, reducing the need for computing power to introducing more components to access control.

\item The transportation and healthcare domains involve many sensitive data. When we design the access control schemes in the end-edge-cloud architecture in these domains, the privacy-preserving methods should be considered thoroughly.  

% \item 
% In terms of PRE, this survey mainly introduces the methods to protect the privacy of data owners and consumers, achieve more fine-grained re-encryption, and accomplish re-encryption more efficiently. 
% In edge computing, data security is complex, and the existing solutions cannot deal with the complexity in practice.
% We should comprehensively consider the ABE\&PRE to make high-performance coarse-grained and fine-grained re-encryption, while effectively resolving the privacy issues in PRE. 

\end{itemize}


\begin{table*}[]
\centering
\caption{Comparison among access control schemes in edge computing from data usage}
\label{Table::DataUsage}
\begin{tabular}{|c|c|c|c|c|p{4.2cm}|c|c|}
\hline
Scheme & Centralization & Obligation & Purpose & Monetization &  \multicolumn{1}{c|}{Granularity} &Requirements & Application  \\ \hline
\cite{cao2020policy}  &  \checked  & \checked  & \checked & \checked &   Spatiality, Temporality, and Aggregation       & \textbf{RU1}\&\textbf{RU2}  & Smart cities \\ \hline
\cite{munoz2020data}  &  \checked &  \checked  &   \checked &  \checked  & Temporality and Aggregation  & \textbf{RU1}\&\textbf{RU2} & Food industry \\ \hline
\cite{kelbert2018data} & - &   \checked      &     -       &      -   &   Temporality       & \textbf{RU1}\&\textbf{RU2} & General \\ \hline
\cite{cirillo2020intentkeeper} &    -    &    -     &   \checked     &  -     & Temporality  &  \textbf{RU1}\&\textbf{RU2} & Automotive industry \\ \hline
% \cite{cao2015usage}  &  \checked & \checked & \checked &   -      &     Spatiality, Temporality    & - & Smart cities  \\ \hline
\cite{xue2022sparkac} & \checked  &  -  &   \checked    &  -   &  Temporality and Aggregation & \textbf{RU1}\&\textbf{RU2} &  General \\ \hline
\cite{arora2022higher} & \checked  &  -  &   \checked    &  -   & - & \textbf{RU1}\&\textbf{RU2} &  General \\ \hline
% \cite{carminati2016enhancing} & \checked &  - & \checked &     -    &   Aggregation       & Single PC & Fitness IoT  \\ \hline
\end{tabular}
\end{table*}

\section{Access control in data usage}

\label{Sec::ACInDataUsage}


After the access control mechanisms in data collection and storage grant access to data, their responsibility for protecting data would end. However, some data owners could expect to learn about how their outsourced data is used and control their data usage.
Data usage control could ensure data sovereignty for data owners.
% In data usage control, reference monitors are expected to monitor the usage of protected data by intercepting system information (e.g., a query tree). This means that the data user's computing systems (e.g., Apache Spark \cite{zaharia2016apache} and Apache Flink \cite{carbone2015apache}) should be interposed by the reference monitors. 
%The studies \cite{lazouski2010usage, nyre2011usage, akaichi2022usage} survey the usage control from various aspects: specification, enforcement, and robustness.
%Purpose-based access control is designed to ensure that access to sensitive or confidential data is only granted when the purpose of the access is consistent with the authorized use of the data.
We next present the recent efforts in DUC.
%from general DUC, purpose-based access control, to TEE-enabled usage control.

% The access
% control requirement is copied from Section III and pasted:
% \textit{Data owners could expect to learn about how their outsourced data is used and control their data usage.
% However, the above access control technologies in data collection and storage would end their responsibility for protecting data after data access is granted. Data usage control could satisfy the requirements of data sovereignty (\textbf{RU1} \& \textbf{RU2}).}


Generally, DUC involves centralized and decentralized implementations. 
Cao et al. \cite{cao2020policy} implement a centralized data usage platform for smart cities, where data usage is restricted by data providers, data monetization is allowed, various obligations are considered, and the used/processed data can be visualized. Therein, the user's role can be used for authorizing data monetization (RBAC). As shown in experiments, the end-to-end delay, i.e., the time from processing the data consumer request to getting the data response, is increased by 42 ms on average. The time of processing usage control is increased by 36 ms on average.  Similarly, Munoz-Arcentales et al. \cite{munoz2020data} present a centralized implementation of DUC for securing data sharing among multiple organizations in the industry. 
Kelbert et al. \cite{kelbert2018data} formalize, implement, and evaluate a fully decentralized system of DUC, where data flow can be tracked, and data usage policies can be propagated and enforced effectively. The assessment indicates that 1) dataflow tracking and policy propagation achieve 21\%–54\% of native execution throughput, and 2) decentralized policy enforcement generally outperforms centralized methods.
% To improve the policy quality, Gonzalo et al. \cite{CAPA4DUC} propose a context-aware policy analysis algorithm to detect the inconsistencies and redundancies in DUC policies. 


Traditionally, the DUC mechanism pre-defines data usage pipelines across domains, e.g., IoT-generated data is outsourced to edge servers for advanced analysis. However, this fashion complicates the process of DUC policy specification, especially when the data usage pipeline is mutable. The existing DUC  techniques cannot preventively and proactively enforce data usage control.
Cirillo et al.
\cite{cirillo2020intentkeeper} propose a practical distributed DUC framework IntentKeeper based on the open-source IoT edge computing framework FogFlow \cite{cheng2017fogflow}. It decouples data usage flow with data usage policy and allows users to specify DUC policy easily using an ODRL-like model \cite{ODRL}. And, it supports preventive and proactive enforcement by federated service orchestration and access control data management. Use case validations demonstrate that IntentKeeper reduces the complexity of policy specification by up to 75\% in moderately complex scenarios, compared with current flow-based approaches. Additionally, experimental results indicate that IntentKeeper ensures rapid response times (under 40 ms) with minimal overhead (below 10 ms).

% In addition, some efforts \cite{cao2015usage, truong2016leverage, denis2021bringing, munoz2019architecture} try to propose data usage control for IoT, where data usage policies are considered from obligations to various constraints, and the non-repudiation of data usage is involved.


% Dang and Hoang \cite{dang2017data} also enforce the fog-based privacy-aware RBAC model after building trust. 
% This model can implement cross-domain data access control according to region, location, the roles of data users, and the purpose of data access, meanwhile obligation(s) can be defined. 

To enforce access control on the general big data computing platform, Spark, Xue et al. \cite{xue2022sparkac} propose purpose-aware access control by enhancing purpose-based access control with data operation/processing purpose (describing the fine-grained data usage). They implement purpose-aware access control in the execution and optimization layers. As a result, the SQL query, machine learning algorithm, streaming computation, and graph computation can be automatically supported by this solution, meanwhile introducing acceptable latency for big data analytics. The fine-grained purpose and the implementation methodology can be adapted for other data analytics at the edge. 
In addition, IntentKeeper \cite{cirillo2020intentkeeper} supports vehicle analytics-related purposes for enforcing DUC.
% Cao et al. \cite{cao2015usage} propose a data usage model for smart cities, where data usage purpose is one of the components, and implement accountability of policy enforcement and traceability of data usage. Carminati et al. \cite{carminati2016enhancing} propose a purpose-based scheme to enhance the users' control of their personal data usage. This scheme makes clear categories of data in the fitness IoT applications, pre-defines a set of data usage purposes, and allows data owners to have fine-grained control of raw data and the derived data according to data categories and usage purposes. 

Arora et al. \cite{arora2022higher} use the higher-order relationship context information to control data usage in the dynamic environment in IoT applications. This scheme uses the history of relationship changes to make authorization decisions. This means that the relationship temporality should be considered. For example, if a nurse has already used the medical data of Alice for care, this nurse cannot use the medical data of Bob for medical research purposes. The proposed graph-matching algorithms for authorization are effective and efficient as shown in the experiments when temporality is introduced into ReBAC.

% \begin{table*}[]
% \centering
% \caption{Comparison among access control schemes in edge computing from data usage}
% \label{Table::DataUsage}
% \begin{tabular}{|c|c|c|c|c|p{4.2cm}|c|c|}
% \hline
% Scheme & Centralization & Obligation & Purpose & Monetization &  \multicolumn{1}{c|}{Granularity} &Testbed & Application  \\ \hline
% \cite{cao2020policy}  &  \checked  & \checked  & \checked & \checked &   Spatiality, Temporality, and Aggregation       & Single PC & Smart cities \\ \hline
% \cite{munoz2020data}  &  \checked &  \checked  &   \checked &  \checked  & Temporality and Aggregation  & FIWARE & Food industry \\ \hline
% \cite{kelbert2018data} & - &   \checked      &     -       &      -   &   Temporality       & Self-built cluster & General \\ \hline
% \cite{cirillo2020intentkeeper} &    -    &    -     &   \checked     &  -     & Temporality  &  FogFlow & Automotive industry \\ \hline
% % \cite{cao2015usage}  &  \checked & \checked & \checked &   -      &     Spatiality, Temporality    & - & Smart cities  \\ \hline
% \cite{xue2022sparkac} & \checked  &  -  &   \checked    &  -   &  Temporality and Aggregation & Self-built cluster &  General \\ \hline
% % \cite{carminati2016enhancing} & \checked &  - & \checked &     -    &   Aggregation       & Single PC & Fitness IoT  \\ \hline
% \end{tabular}
% \end{table*}




\textit{Summary and Lessons Learned:}
In this section, we have discussed the studies to satisfy
\textbf{RU1}\&\textbf{RU2}. The approaches are summarized in Table \ref{Table::DataUsage}, and the learned lessons are as follows:
% \begin{itemize}
%     \item 
%As shown in Table \ref{Table::DataUsage}, we summarize the access control solutions from the following aspects: centralization, obligation, purpose, monetization, granularity, testbed, and application.
Most schemes focus on a specific application realm to implement centralized DUC by building the corresponding purpose set. 
Obligation is considered in most DUC implementations.
DUC can use monetization to facilitate data flow. 
The granularity of DUC can be divided into three categories: spatiality, temporality, and aggregation. 
Different schemes may involve different granularity.
The purpose component is regarded as the core component for satisfying data owners' privacy in DUC \cite{akaichi2022usage}.  
In purpose-based schemes \cite{byun2008purpose}, data owners specify ``which data users can use data in which purpose''. If the usage purpose indicated by data users complies with the data-owner-specified purpose, the user's query will be allowed to use data. 
Purpose-based schemes control data usage before execution, meaning that the data analysis logic operates on data loaded into memory in processors (e.g., CPU).

% \item 
% During data running, hardware enclave (e.g., SGX \cite{mckeen2013innovative}) acts as the essential component and guarantees data confidentiality and secure execution of computation. Zheng et al. \cite{zheng2017opaque} propose Opaque, which combines SGX with Spark SQL for secure data analytics on the cloud.  
% Sketch algorithms can be used to reduce the communication cost in a wide range of applications (e.g., federated learning) \cite{yang2019federated, konevcny2016federated, jiang2018sketchml}.
% Bagher et al. \cite{bagher2023sgx} introduce SGX-Stream for sketch algorithms in edge-cloud architecture, where the SGX-Stream enclave preprocesses data at the edge and generates sketches, which are sent to the cloud for further processing in the SDX enclave. SGX-Stream achieves a 14x speedup on urgent tasks while using less than 800 KB of scheduling memory. Additionally, its practicality is demonstrated through three real-world applications: network stream, genomics, and website click stream.
% %he existing works generally focus on data protection in static and single scenarios, where different participators (i.e., edge servers and cloud servers) separately enforce purpose-based or hardware-assisted usage control without dynamic interoperations among them. 
% Purpose-based/Hardware-assisted schemes in different edge servers can be cooperated for effective data computation. 
% %\textbf{For example, because enormous computing nodes exist in edge computing, selecting appropriate edge nodes and data upload frequency (from edge to cloud) can execute distributed DUC more efficiently according to network conditions. }
% %Moreover, the real-time data usage policy specification from data owners should be responded to reliably and flexibly.


% \end{itemize}

\section{Blockchain-based access control platform}
\label{Sec::BBACP}
Although the studies in the above sections can be selected for achieving access control, which depends on small resources or has acceptable delay, flexibility, and scalability, they do not consider the security of critical access control data in edge computing.
%: scalability, decentralization, and trust. 
%For example, they cannot avoid the verification because they generally depend on a centralized key generation center in ABE.
In this section, we study how to ensure this security by depending on the advantages of blockchain, i.e., decentralization, immutability, programmability, and security  \cite{dabbagh2021survey, zhang2021resource, zheng2018blockchain}.
%Recently, lots of studies have been conducted to combine blockchain with access control to secure edge computing. 
We introduce the recent blockchain-based access control platforms developed for managing the data of access control in different data lifecycles. In particular, we mainly introduce which typical access control models are combined with blockchain, and the method of exploiting blockchain to manage the data of these models.
%, and the performance of related blockchain-based schemes. 


\subsection{Blockchain-based access control in data collection}

Liu et al. \cite{liu2020fabric} introduce an access control system, Fabric-IoT, which exploits Hyperledger Fabric to manage ABAC used for the resource data generated by IoT devices. They use smart contracts to implement resource access, policy management, and policy enforcement. In particular, the device contract provides methods to store/query URLs of resource data; the policy contract provides functions to manage access control policies; and the access contract enforces access control. 
The simulation experiments present acceptable throughput and efficient consensus. 


Mazzocca et al. \cite{mazzocca2022framh} propose a risk-aware authorization middleware for healthcare based on federated learning. 
Blockchain stores the trained federated model, which evaluates the risk level of the current patient. %Sabrina \cite{sabrina2019blockchain} proposes a structural ReBAC model. 
% It uses smart contracts and a public blockchain to manage access control for external users and uses local off-chain storage to manage access control for users within an organization. 
% External users access IoT resource data based on access control tokens generated by executing smart contracts on the public blockchain. 
Sylla et al. \cite{sylla2021blockchain} propose a new blockchain-enabled decentralized context-aware authorization system. 
Users can dynamically define contextual access rights for each IoT application in smart contracts. 
When an authorized client issues a request, the smart contract generates the corresponding contextual access token. With the edge deployment of blockchain, the maximum generation time of contextual access tokens is about 10 ms. 

In practice, we need the management of capability registration, delegation, and revocation in CapBAC.
The centralized management component likely induces performance bottlenecks and single-failure problems. 
The blockchain can be used for capability registration, delegation, and revocation \cite{liu2021capability, xu2019exploration}.
The blockchain-enabled decentralized CapBAC (BlendAC), which is being researched in the academic community, can avoid those problems. 
Xu et al. \cite{xu2018blendcac} propose a BlendAC for large-scale IoT systems. It achieves robust identity-based capability token management, where the smart contract is used for registration, validation, delegation, and revocation. They implement BlendAC on a Rasberry Pi device and on a local private blockchain. The experimental results demonstrate that BlendAC can offer decentralized, scalable, lightweight, and fine-grained access control.
Similarly, the following studies design the blockchain platforms based on CapBAC, where different capability tokens are considered.
IoT consortium capability-based access control (IoT-CCAC) \cite{bouras2021iot} utilizes blockchain to achieve decentralized CapBAC schemes for consortium applications in IoT cities, where IoT-generated data from different parties is governed for different services by using group capability tokens.
Nakamura et al. \cite{nakamura2020exploiting} propose a novel CapABC scheme, where the smart contract is used for managing the tokens that each combines with an action and are different from the conventional token model, i.e., one token per subject. This solution allows subjects to have multiple tokens and facilitates flexible token delegation among multiple subjects. Chen et al. \cite{chen2023capability} present a fine-grained and flexible access control scheme, which simultaneously achieves flexible capability granting and revocation, sufficient capability granularity, secure capability delegation, and capability verification. This scheme combines blockchain with CapBAC, where a smart contract manages subject and object information.
%and achieving operations (e.g., capability revocation). 
It designs authorization rules and a tree for capability, where the token considers context information.



% To secure data sharing in edge-cloud collaboration, Sun et al. \cite{sun2022blockchain} propose a protocol based on ABE. This solution supports privacy protection by hiding attributes of terminals, provides cross-domain access control for cross-domain data sharing among terminals, incorporates dynamic access control for intermittent terminals, and achieves fine-grained access control by combining attributes. Therein, the dynamic access permissions can be updated on a blockchain.


\subsection{Blockchain-based access control in data storage}
Considering the difficulty of deploying the existing blockchain platforms, Zhang et al. \cite{zhang2021lightweight1} design a lightweight blockchain (LBC) by improving the proof-of-work consensus for lightly implementing blockchain. Moreover, they use blockchain to store access control policy to protect the privacy of policy and design six smart contracts for integrating ABAC and ABE. 
In particular, the policy management contract (SCPA) operates the policy set and generates encryption policies; the policy decision contract determines the policy compliance according to policies from SCPA; the policy information contract manages attribute information for SCPA; the encryption and decryption contract enforces ABE by edge nodes; the penalty mechanism contract manages the punitive measures for illegal access; the policy enforcement contract returns the encrypted data or available resources.
Attribute updates/revocations in ABE are incompatible with the immutability of blockchains.
To address this issue, Yu et al. \cite{yu2020enabling} propose a new blockchain-based access control for IoT systems, which allows attribute updates/revocations by integrating Chamelon Hash (CH) algorithms into blockchains. To ensure the security of key updates, they further design a key chain for verifying key updates to avoid the abuse of CH update function.
However, these works do not consider the privacy preservation of user data. Han et al. \cite{han2021blockchain} propose a blockchain-based auditable access control system for private data in IoT. Based on the ABAC model, they define a model to divide the IoT data into private data and public data and utilize smart contracts for storing and managing the private data, access control policy, and access records. 
In the smart grid area,
Yang et al. \cite{yang2020secure} present a blockchain-based CP-ABE access control system for smart grid, where amounts of data generated by IoT devices need to be shared among distributed energy resources, microgrids, and the main grid. The blockchain is combined with edge computing, where the partial encryption/decryption tasks of CP-ABE are executed in the form of smart contracts. 
%Moreover, this work addresses the single point of failure problem in  the centralized authority scenario by utilizing the (\textit{t},\textit{n}) threshold secret sharing scheme. 

% To improve PRE, Manzoor et al. \cite{manzoor2021proxy} propose a blockchain-based PRE scheme, which implements decentralized data sharing by blockchain. In this PRE scheme, the data is visible to users on the smart contracts. Agyekum et al. \cite{agyekum2021proxy} present a similar scheme, but identity-based encryption is used for fine-grained access control.
% Chen et al. \cite{chen2020blockchain} propose another blockchain-based PRE scheme, which considers the searchable encryption and equality test for ciphertext. 
% Chen et al. \cite{chen2021threshold} describe a threshold scheme, where trusted multiple proxy nodes are used for re-encrypting ciphertext.


\subsection{Blockchain-based access control in data usage}
IntentKeeper \cite{cirillo2020intentkeeper} uses Hyperledger Fabric to propagate, synchronize, and record some important data, e.g., data usage policies, distributed sites, and policy enforcement decisions.
Syed et al. \cite{syed2020novel} design a blockchain-based vehicle lifecycle tracking framework, where Hyperledger Fabric enables the DUC engine to monitor vehicle maintenance, insurance, and rented vehicles continuously (e.g., restriction on the number of vehicle leases). Specifically, they develop smart contracts for enforcing DUC and maintaining DUC policy.
Wu et al. \cite{9662435} present the TS-PBAC model, which leverages blockchain-enabled secure logs to evaluate quality data from the external network. This model allows individual-centric privacy preservation in the Internet of Medical Things scenarios, where medical data can be specified for different purposes by data owners. Meanwhile, local differential privacy and RBAC are combined to protect sensitive attributes against internal users. 
To mitigate the trust and security problem for IoT big data management, Ma et al. \cite{zhaofeng2019blockchain} propose a BlockBDM scheme, where public and permissioned blockchain is utilized for performing data operations and their management. In particular, BlockBDM achieves secure usage control by limiting the operations (e.g., data backup and data save) and recording data usage for auditing trails. 
These studies \cite{xiao2020privacyguard, zhang2021data, pol2021preserving,gao2021blockchain,han2022blockchain} combine trusted execution environment (TEE), e.g., SGX, with blockchain. The smart contract is used to manage data usage policies and data trading prices. Controlling data usage is achieved by a TEE-based off-chain contract execution engine, and the results are securely committed to the blockchain for the auditing trail.  


\subsection{Blockchain-based versatile access control platform}
A blockchain-based versatile access control platform can provide multiple access control implementations, which intends to be used for multiple data lifecycles.
Implementing a useful versatile access control platform is tricky because data and services are complicated in edge computing, the application scenarios cannot be pre-known, and on-chain data is costly \cite{international2018new}. 
Focusing on the smart contract-based access control (SCAC), Zhu et al. \cite{zhu2022fine} explore how to combine blockchain security with fine-grained access control models while keeping the efficiency of edge computing. SCAC depends on ABAC and RBAC to develop basic entities in the model of SCAC, including attributes (e.g., token and identity), smart contracts (e.g., register manager and device, set attribute predicate, and query information). 
Ouaddah et al. \cite{ouaddah2016fairaccess} present a blockchain-based access control framework FairAccess to enable its users to own and control their data. It uses a public Bitcoin-like blockchain to act as the access control manager, which supports various access control models (e.g., RBAC and ABAC) and transactions (grant, get, delegate, and revoke access). In \cite{ouaddah2021fairaccess2}, they update FairAccess to FairAccess2, where more granular data access control policies are supported based on Ethereum. Based on Ethereum, Oscar et al. \cite{novo2018blockchain} propose a decentralized access control system for the IoT. This system utilizes blockchain technology to store and distribute access control information, and it supports resource-constrained devices. A single smart contract is designed to enforce access control based on the access control policy of a set of IoT devices, where a manager is supervised to manage these devices. However, this access control approach is too complex for changing permissions and cannot fully meet the dynamic requirements of the IoT.
% Zhang et al \cite{zhang2018smart} propose another framework for IoT, where one access control contract (ACC) defines one access control method based on static access control policy, and meanwhile judge contract dynamically validates ACC by evaluating subject behavior, register contract registers access control information, misbehavior-judging method and corresponding smart contract, and provides operations (e.g., register and update). 
Zhang et al. \cite{zhang2018smart}  present a novel framework for the IoT that centers around Access Control Contracts (ACCs). In this framework, each ACC is responsible for defining a specific access control method based on a static access control policy. Simultaneously, a Judge Contract dynamically evaluates the ACCs by assessing the behavior of subjects registered in the system. The Register Contract records access control information, misbehavior-judging methods, and the associated smart contracts, offering functionalities such as registration and updates. This approach provides a structured and dynamic means of managing access control within IoT environments.


\subsection{Summary and lessons learned}
In this section, we have discussed the studies applying blockchain to protect important access control data while satisfying \textbf{RC1}\&\textbf{RC2}, \textbf{RS1}\&\textbf{RS2}, or \textbf{RU1}\&\textbf{RU2}. 
%As a commonplace infrastructure, blockchain technology can be used to protect the critical access control data. 
%As shown in Table \ref{Table::BlockchainForAC}, we summarize some blockchain-based schemes with four categories: blockchain for access control in data collection, blockchain for access control in data storage, blockchain for access control in data usage, and blockchain for versatile access control platform. 
%We show the comparison from the following aspects: blockchain, supported model, and operation. 
The approaches are summarized in Table \ref{Table::BlockchainForAC}, and
the learned lessons are as follows:


\begin{table*}[]
\centering
\caption{Comparison among blockchain-based access control schemes in edge computing for data collection, storage, and usage}
\label{Table::BlockchainForAC}
\begin{tabular}{|p{2cm}<{\centering}|p{0.8cm}<{\centering}|p{2.5cm}<{\centering}|p{3.4cm}<{\centering}|p{7cm}|}
\hline
Lifecycle                                 & Scheme               & Blockchain         & Supported model(s) & Operations                                                                                             \\ \hline
\multirow{5}{*}{Data collection}      & \cite{liu2020fabric}             & Hyperledger Fabric & ABAC               & Policies CRUD, policies enforcement, resource URLs CRUD                                                \\ \cline{2-5} 
                                      & \cite{mazzocca2022framh}             & Ethereum & RAAC               &  Stores the trained federated model
                                              \\ \cline{2-5} 
                                      % & \cite{sabrina2019blockchain}             & Ethereum & ReBAC/CapBAC               & Access token register, validation, delegation, and revocation, according to relationship                                               \\ \cline{2-5} 
                                      & \cite{sylla2021blockchain}             & Hyperledger Fabric/Ethereum & CAAC/CapBAC              & Context token register, validation and revocation                                               \\ \cline{2-5} 
        &\cite{xu2018blendcac}             & Ethereum           & CapBAC             & Identity token register,validation, delegation, and revocation                                         \\ \cline{2-5} 
                                      & \cite{bouras2021iot}             & BigchainDB         & CapBAC/GBAC             & Group token register,validation                                                                        \\ \cline{2-5} 
                                      & \cite{nakamura2020exploiting}            & Ethereum           & CapBAC             & Action token register, validation, delegation, and revocation                                           \\ \cline{2-5} 
                                      & \cite{chen2023capability}            & Hyperledger Fabric & CapBAC/CAAC             & Token register, validation, delegation, and revocation                                          \\ \hline
\multirow{4}{*}{Data storage} & \cite{zhang2021lightweight1}  & LBC                & CP-ABE/ABAC      & ABAC policy CRUD, and encrypting/decrypting data or policy file by CP-ABE                              \\ \cline{2-5} 
                                      & \cite{yu2020enabling}                   & -                & CP-ABE             & Attributes update/revocation                                                                                     \\ \cline{2-5} 
                                      &  \cite{han2021blockchain}                   & Hyperledger Fabric & ABAC               & Upload/Query private data and URLs of public data, Update/Query access record, Policy CRUD             \\ \cline{2-5} 
                                      & \cite{yang2020secure}   & Hyperledger Fabric & CP-ABE             & Data owners and data users can use smart contracts to accomplish partial data encryption and decryption \\ \hline
\multirow{2}{*}{Data usage}        & \cite{cirillo2020intentkeeper}  & Hyperledger Fabric & DUC               & Upload/Query data usage policies, distributed sites, policy enforcement decisions.                     \\ \cline{2-5}
                                      &  \cite{syed2020novel}        & Hyperledger Fabric & DUC                & Upload/Query data usage policies and attributes, DUC enforcement engine                                \\ \cline{2-5}
                                       &  \cite{9662435}        & ChainSQL & DUC                & Record EMR records, model parameters of access control, privacy policies, and access logs. Enforce PBAC                                \\ \cline{2-5}
                                       & \cite{zhaofeng2019blockchain}          & Hyperledger Fabric  & DUC                & Limit the number of uses, the period of use, backups, etc.                                \\ \hline
\multirow{2}{*}{Multiple lifecycles}        & \cite{zhu2022fine}  & Hyperledger Fabric  & RBAC and ABAC               & Register manager and device, set attribute predicate, query information, etc.                     \\ \cline{2-5}
                                      &  \cite{ouaddah2016fairaccess, ouaddah2021fairaccess2}        & Modified Bitcoin, Ethereum&  RBAC, ABAC, etc.               & Grant, get, delegate and revoke access                                \\ \cline{2-5}
                                       &  \cite{novo2018blockchain}        & Ethereum & General architecture for resource-constrained devices  &  Register manager and device, add and remove manager, add access control enforcement, revoke permission, etc.                             \\ \cline{2-5}
                                       & \cite{zhang2018smart}          & Ethereum  & General architecture for resources access in IoT                & Register
access control information, misbehavior-judging method and
corresponding smart contract, and provides operations (e.g.,
register and update)                               \\ \hline
\end{tabular}
\vspace{-0.1cm}
\end{table*}


\begin{itemize}
    \item 
In data collection, many studies focus on utilizing blockchain technology to optimize traditional CapBAC by implementing decentralized CapBAC. The smart contract generally accomplishes operations on tokens in CapBAC. 
As lessons learned in Section \ref{Sec::SALInDataCollection}, the tokens in CapBAC are often incorporated with some components (e.g., trust and group).
%the existing work mainly resolves a specific problem in data collection by combining CapBAC and other access control models. 
As such, it would be interesting to build a blockchain management system, which can provide a library of various tokens for complex edge computing applications.

\item 
%\textbf{
In data storage, blockchain can be used to manage access policies in ABE, execute computing in ABE, record access permissions, etc. Depending on a blockchain, we can integrate ABAC and ABE securely while achieving flexible and scalable access control.
%Blockchain can manage the data users and data providers in PRE, guarantee the quality of ciphertext from PRE, and construct distributed and trusted proxies. 
%However, the blockchain is explored separately for implementing a secure access control system based on ABE and PRE. 
%In particular, the foundational components for data encryption/decryption (e.g., attribute, policy, key management, and proxy) are separated.
%In the edge computing scenario, the separated components in ABE and PRE should be integrated or organized from the perspective of an edge computing access control system to implement practical data cryptography for access control. }

\item 
Blockchain in each DUC scheme is generally used as a platform to regulate data usage rules, guarantee the consensus of executing data usage rules, and record model parameters and data usage records.
Purpose-based schemes generally request data users to input their data usage purpose. 
In this fashion, malicious users may cheat purpose-based enforcers. 
Relational audits can deter data users from being dishonest if the purpose-based schemes are integrated into blockchain to manage purpose.

\item 
From the blockchain for access control in data collection, storage, and usage, we can observe that each data phase has a limited number of blockchain-supported models. 
%Each blockchain-based scheme is designed for specific scenarios separately. 
Given the intricate and dynamic nature of the access control requirements, each data phase should be equipped with a sufficient range of blockchain-supported models.
In addition, we observe that the access control schemes in each data phase have common components, such as model parameters management, policy CRUD, access logs record, attributes CRUD, model enforcement, etc.
We could design a lightweight blockchain-based versatile access control platform depending on these common components.
Finally, these blockchain-based approaches are crafted for distinct scenarios individually, involving Hyperledger Fabric, Ethereum, ChainSQL, etc.  
If each separated blockchain in each data phase integrates appropriately, it could induce extra overhead, such as communications between different access control systems of multiple data phases, and prevent access control performance from being improved in edge computing.
%From the perspective of the whole access control system of edge computing, the current tanglesome access control solutions can complicate access control management, which goes against the data security in edge computing. And, if each separated blockchain in each data phase has no appropriate integration with each other, it could induce extra overhead (e.g., communications between different access control systems of different data phases) and prevent the performance of access control from being improved in edge computing. Finally, it is common for different blockchain systems to be explored in practice. 
The interaction among different blockchains should be supported for access control systems. 


\item 
Blockchain can support multiple access control models for multiple lifecycles, where smart contracts enable various operations: register access control enforcement, manage attributes, etc. 
Versatile access control technology could be the feasible solution to solve the data security problem in edge computing, which has various stakeholders, ample data sources, diversified dynamics, and complex applications. However, the current blockchain-based versatile access control platforms mainly support conventional models (e.g., ABAC, RBAC, and CapBAC), and lag the development of new techniques as introduced in Section \ref{Sec::ACInDataCollection}\&\ref{Sec: ACInDataStorage}\&\ref{Sec::ACInDataUsage}, where the improvements for conventional models are designed.


\end{itemize}






==> Tex/Access_Control_Requirement.tex <==
% \begin{figure}
% 	\begin{center}	\includegraphics[scale = 1.7]{AllFigures/edgeservices.pdf}
% 		\caption{Edge computing services.}
% 		\label{Fig::EdgeServices}
% 	\end{center}
% \end{figure}



\section{Edge Computing and Requirements Analysis on Access Control}
\label{Sec::RAoAC}




\subsection{Edge Computing}
\label{Sec::Background_EdgeComputing}

 



Traditionally, the central cloud is the main platform to provide computing power for a wealth of data from distributed heterogeneous IoT devices \cite{botta2016integration}. 
The traditional cloud-centric architecture involves long propagation delays, which is unacceptable for latency-sensitive applications \cite{lim2020federated}. 
We can find some latency-sensitive examples in \cite{varghese2016challenges}. For example, in a smart health system, a large amount of data generated by smart sensors for telemedicine needs to be processed in microsecond latency. 
In the telemedicine scenario, the high-solution videos need to be shown to doctors in time.
A visual guiding service using a wearable camera requires a preferred response time between 25 ms to 50 ms.
%In the mobile scenario, video streaming is the largest mobile traffic generator and it will not satisfy the users' low-delay experiences if the bulk of this traffic is channeled to the same source \cite{jiang2021survey}.
%Similarly, multimedia applications, such as on-demand gaming on current cloud infrastructure, pose similar latency issues for the gamer \cite{varghese2016challenges}. 



%Edge computing mitigates the challenges and attracts the attention of the academic and industrial community. 
To conquer the latency challenges in traditional cloud computing, the end-edge-cloud system architecture, as shown in Figure \ref{Fig::EdgeComputing}, is proposed with these layered and connected components: cloud, edge nodes, and end devices \cite{shi2016edge}, where data can be processed closer to the data source. 
In particular, edge nodes connect with pervasive heterogeneous IoT devices, and interact with the cloud, meanwhile, an edge computing orchestrator could orchestrate cooperative work among edge nodes/cloud \cite{ren2019survey}. 
%, and dispense content in the vicinity of user equipment.
Massive data collected from IoT devices can be aggregated at edge nodes distributedly before the data is delivered to the cloud. Real-time data processing and basic analytics can be fulfilled at the edge.
Due to the advantages of edge computing, it has been widely used in many applications as shown in Figure \ref{Fig::EdgeComputing}, including smart transportation, smart sea monitoring, smart homes, smart health, etc.

\begin{figure}
	\begin{center}
	\includegraphics[width=\columnwidth]{AllFigures/EdgeComputingArchitecture.pdf}
		\caption{The end-edge-cloud system architecture \cite{shi2016edge}.}
		\label{Fig::EdgeComputing}
	\end{center}
\end{figure} 


% Next, we further present several advantages apart from the low latency above \cite{bonomi2012fog}, including data privacy, flexibility, and predominance of wireless access.
% Note that we analyze the requirements for access control by considering the challenges from these advantages in the next section. 

% \textit{Data privacy:} Traditional cloud computing requires large raw data to be centrally uploaded to the cloud for unified processing, which increases the risk of data loss and leakage \cite{cao2020overview}. 
% However, edge computing enables data to be processed locally by deployed edge servers, reducing the need to transfer data to the cloud for processing, thus enhancing data privacy and security. 
%By leveraging various techniques, such as data encryption and data masking \cite{liu2019survey}, edge computing can further enhance the confidentiality and security of sensitive data. 

% In terms of energy consumption, there is a significant number of research on cloud data centers \cite{dayarathna2015data}. 
% Data centers in the next decade are likely to consume three times as much energy as consumed today \cite{EnergyComsumption}.
% Compared with traditional cloud computing, edge computing has obvious advantages for saving energy. 
% Due to fewer data transfers, network bandwidth is saved, the network bandwidth load is unburdened for the cloud, and the energy consumption is greatly reduced. 
% Due to the limitations of energy and computing resources, low-energy chips and algorithms are thrust into edge computing \cite{EssentialsofEC}.


% \textit{Flexibility:} Application scenarios continue to change and evolve \cite{taleb2017multi}. In particular, unbound IoT devices may be added; short-lived interaction is typical; IoT data consumers are potentially changing. 
% The demands on computing resources are various. The decentralized architecture of edge computing enables to allocate of computing resources more dynamically and flexibly.
% Resources are used more efficiently, and computing tasks are performed in a timely and cost-effective manner. 


% In many IoT application scenarios, different wireless communication protocols are required to transmit IoT data 
% \cite{khan2019edge, EssentialsofEC}. 
% For example, WiFi has high-speed connectivity and has been widely used in homes and offices. 
% Bluetooth can achieve low-energy communication and enable long lifetimes for battery-operated devices. 
% The fifth generation of wireless technology (5G) provides bigger broadband, lower latency, and massive machine-type communication. 
% These wireless communication technologies are used in many areas. 
% For example, Bluetooth protocols are used by wearable devices for communicating with phones in healthcare scenarios. 
% 5G is used by environment monitoring sensors for communicating with the base stations in agriculture and industry scenarios.
% Edge computing seamlessly combines with these wireless communication technologies to facilitate wireless connection and data transmission of devices and applications.


\subsection{Requirements Analysis on Access Control}

 
This section would describe the access control requirements for edge computing in the tri-layer end-edge-cloud architecture.
%Data security is immanently enhanced in edge computing because data can be processed locally within some security zone and data transit is reduced in the network. 
Traditional cloud computing requires large raw data to be centrally uploaded to the cloud servers for unified processing, which increases the risk of data loss and leakage \cite{cao2020overview}. 
However, edge computing enables data to be processed locally by deployed edge servers, reducing the need to transfer data to the cloud servers for processing, thus enhancing data privacy and security. 
With massive data processed at the edge, access control, as the common fundamental technique for protecting data, should be studied thoroughly. 
To have a clear analysis of access control requirements, we first show the following natural characteristics of edge computing, which would challenge the access control at the edge \cite{xiao2019edge, khan2019edge}:
\begin{itemize}
\item 
\textit{Limited resources:} As shown in Figure \ref{Fig::EdgeComputing}, various smart devices are at the end. However, these devices often have constraints on resources (e.g., energy, storage, computation, and communication), while executing access control generally requires enough resources.

\item 
\textit{Low latency:} Edge computing embodies latency-sensitive applications. In particular, the latency in edge computing includes many aspects: task-offloading time, communication latency, computation cost, security-induced cost, etc. \cite{liu2019dynamic, kai2020collaborative}.
The total of these delays should be as small as possible.
%The delay from an access control mechanism should be . 
The low latency of edge computing should not be negated by those aspects. 

\item
\textit{Flexibility:}
Data producers and consumers are generally dynamic. In particular, unbound IoT devices may be added; short-lived interaction is typical; services are potentially changing \cite{khan2019edge}. As such, the dynamic nature of data producers and consumers in edge-computing scenarios necessitates flexibility in security measures to accommodate this dynamism.

\item
\textit{Scalability:} The decentralized architecture of edge computing allocates computing resources at scale  \cite{khan2019edge}. In this way, the widespread geographical distribution of edge nodes would naturally challenge the scalability of centralized security mechanisms and complicate trust management in such a decentralized environment.
%In the largely geo-distributed edge nodes, traditional centralized access control has limited scalability, and trust is difficult for management. 

\end{itemize}

\begin{figure}
	\begin{center}	\includegraphics[width=\columnwidth]{AllFigures/AccessControlRequirements.pdf}
		\caption{Access control requirements analysis in edge computing.}
		\label{Fig::DataACRE}
	\end{center}
\end{figure}

Corresponding to the above characteristics of edge computing, the access control of edge computing should depend on small resources and have low delay, flexibility, and scalability. The typical models and blockchain technology introduced in Section \ref{Sec::TraAccessControl} can be used to satisfy the requirements. Specifically, we would analyze how to satisfy these requirements in this survey from the perspectives of the following common data lifecycles: data collection, data storage, and data usage \cite{DLM}.

To clarify the requirements analysis, we first generalize the basic process of service provisioning and utilization in the tri-layer end-edge-cloud architecture according to the studies \cite{wang2020convergence, fan2021serving, bozorgchenani2018centralized}. 
%In the development of edge computing, services at the edge are developing  
Figure \ref{Fig::DataACRE} (I) shows four kinds of stakeholders in edge computing services: users, service providers, edge computing providers, and cloud computing providers \cite{ning2020distributed}. 
Generally, service providers register on the cloud  (\textcircled{a}), and cloud computing providers authorize corresponding services on legal edge servers (\textcircled{b}). 
Then, users register services from service providers(\textcircled{c}), and users can get registered services from edge servers of edge computing providers (\textcircled{d}).
In this paper, IoT devices and edge services act as various users. 
To describe the access control requirements, we generalize three kinds of services here, i.e., data collection service, data storage service, and data usage service (as shown in Figure \ref{Fig::DataACRE} (II)), which correspond to each data lifecycle respectively. 





%We summarize the kinds of reviewed access control solutions in Table \ref{Table::ACReuqirementsTable}.




\textit{Data Collection:} 
%First, we consider the access control of data collection from IoT devices %edge services, and from the collaborations among edge/cloud nodes. 
% We will present recent efforts in Section \ref{Sec::ACOnServices}. 
As shown in Figure \ref{Fig::DataACRE} (II), IoT devices generate large amounts of data. 
Because IoT devices commonly have limited computation and storage resources or some services require various data from IoT devices, IoT-generated data is uploaded to edge servers for the related services. In particular, as shown in the green box in Figure \ref{Fig::DataACRE} (II), \ding{172}\ding{174}arrows indicate the end$\rightarrow$edge data collection, i.e., collecting data to use it at edge; \ding{173} arrow indicates another end$\rightarrow$edge data collection, i.e., collecting data to store it at edge.
In the process, access control should determine which IoT-generated raw data can be accessed by which services, meanwhile the access control should be flexible given the flexibility of end devices and services (denoted as \textbf{RC1} requirement). 
%The following traditional access control techniques can be used. 
%ACLs control which data is selected. 
The following access control models can be used for satisfying \textbf{RC1}: GBAC, ABAC, CapBAC, and CAAC. Therein, GBAC can facilitate data management by leveraging the group concept on IoT devices. 
ABAC could be suitable because it can adapt the across-domain data collection.
CapBAC consumes small resources of IoT devices due to its method of authorization of access rights. CAAC can use basic context and derived context information to further accommodate the flexibility of edge computing.
%要考虑低延迟、灵活性、扩展性


% The uploaded data should prove that the service can access it.
% Due to the subject-oriented authorization, CapBAC has many advantages in adapting to the dynamic environment of edge computing. 
% For example, it externalizes and distributes the authorization process, and avoids complex and dynamic subject identity management, as well as allows users to store small size of access control policies. 
% The high-performance implementation of CapBAC for the enormous amount of IoT devices is expected. 
% Data cryptography can be combined to guarantee the confidentiality of the transmitted data. 


Due to the end-edge-cloud architecture, as shown in Figure \ref{Fig::DataACRE} (II), data collection from edge to cloud or from edge to edge is commonplace \cite{wang2020edge}. In particular, as shown in the green box in Figure \ref{Fig::DataACRE} (II), \ding{175} arrow indicates the edge$\rightarrow$edge data collection, i.e., some data usage services produce intermediate aggregation results, and data storage services may collect them to store them. 
\ding{176}\ding{177}\ding{178} arrows indicate the  edge$\rightarrow$cloud data collection, i.e., edge computing could achieve real-time data processing while cloud services collect/sample some data at the edge for further advanced analysis.
%However, the results are likely unreliable because vulnerable or malicious edge nodes may tamper with data or transfer fake data. Moreover, compromised edge nodes could transfer normal data, and interfere with the final query results. 
In this situation, access control should determine which intermediate data can be accessed by which edge services
or cloud services (denoted as \textbf{RC2} requirement).
The required access control techniques include CapBAC, ABAC, and CAAC similar to in \textbf{RC1}. Besides, ABE can prevent the collected small raw data from being leaked on malicious edge servers. 
%Moreover, the data collection indicates data is flowing and generally does not require data re-encryption, thus PRE is not considered. 
%ABAC could be suitable because the data collection is not as dynamic as the data collection at the end of IoT devices. %In terms of CapBAC, it reduces the required resources for enforcing access control, but its token management increases the complexity of systems. %The traditional RBAC and ABAC have a trade-off with CapBAC, i.e.,  resource constraints and system complexity. 
%Because edge nodes generally have enough resources, CapBAC is not generally considered in \textbf{RC2}.


\textit{Data Storage:} Second, we inspect the access control for securely storing the IoT-generated data and its related computation results, so that the stored data can be securely used for mining valuable insights or interacting with the IoT devices.
%Figure \ref{Fig::DataACRE} shows that the IoT generates data afterwards edge servers collect, store, and analyze them. 
In particular, due to limited resources on IoT devices, IoT-generated data would be stored on edge servers, as mentioned \ding{173} arrow; and the computation results of IoT-generated data could be stored on edge servers, as mentioned \ding{175} arrow. 
The stored IoT-generated data should be accessed by corresponding authorized parties, which have different access rights to data (denoted as \textbf{RS1} requirement). 
The stored computation results may cooperate among edge servers, where different edge services should access different computation results (denoted as \textbf{RS2} requirement). 


\begin{table*}[]
\caption{Involved typical access control models in each classification in this survey}
\label{Table::ACReuqirementsTable}
\centering
\begin{tabular}{|l|c|c|l|l|c|c|c|c|}
\hline
\multirow{2}{*}{\diagbox{LC}{AC}} & \multirow{2}{*}{CapBAC} & \multirow{2}{*}{RBAC} & \multicolumn{1}{c|}{\multirow{2}{*}{ABAC}}& \multicolumn{1}{c|}{\multirow{2}{*}{ABE}} & \multicolumn{1}{c|}{\multirow{2}{*}{DUC}}& \multirow{2}{*}{GBAC} & \multirow{2}{*}{CAAC (basic, TBAC, RAAC, ReBAC)} &  AC Data Management                                                                                                                                         \\ \cline{9-9} 
                       &                                                &                       &                      & \multicolumn{1}{c|}{}                                      &                       &                       &  &    \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Blockchain for AC in DC\\ Blockchain for AC in DS\\ Blockchain for AC in DU\\ Blockchain as VACP for \\ multiple data lifecycles \end{tabular}} \\
                       \cline{1-8} \xrowht{7pt}
DC                     &  \checked & - & \checked & \checked & -  &  \checked & \checked,\checked,\checked,-  &      \\ 
\cline{1-8} \xrowht{7pt}
DS      &   -    & \checked  &  \checked & \checked &  - &  -                  &   \checked,\checked,\checked,-  &   \\ \cline{1-8} \xrowht{7pt}
DU    &   -    &  \checked  &  -   &  -   &  \checked  & - &  \checked,\checked,\checked,\checked  &                                                                                                                                                    \\ \hline 
\end{tabular}
\vspace{1mm}
 \begin{tablenotes}
     \item[1] AC: Access Control, LC: Lifecycle, DC: Data Collection, DS: Data Storage, DU: Data Usage, VACP: Versatile Access Control Platform
   \end{tablenotes}
\end{table*}

  

Data cryptography for access control is practical for satisfying \textbf{RS1} \& \textbf{RS2}.
Edge servers commonly belong to third parties.
The encrypted data ensures that malicious third-party edge servers cannot peep data easily, meanwhile, the native access control functions by cryptography can control which subject can access which part of encrypted data \cite{di2007data}.
ABE-based access control is promising, where various attributes, e.g., role, context, trust, risk, etc. can be used for regulating access policies flexibly.
Moreover, ABE-based access control has mobility, i.e., each distributed data-hosting party can be a policy enforcement point because the ciphertext of data is combined with the access control. 
It is a data-centric access control without centrally depending on a policy enforcement point. 
ABE could prompt data sharing with high flexibility and scalability in edge computing. 
%Because the multi-authority environment in edge computing is commonplace and different attributes are controlled by multiple parties \cite{chase2007multi}, we should consider the multi-authority ABE (MA-ABE). 
%Because ABE involves resource-consuming data encryption/decryption, implementing high-performance ABE-based access control is essential for edge computing.  




% In a dynamic edge computing environment, data authorization transitions would occur frequently.
% The transition can be achieved by generating new encryption/decryption keys and removing deprecated ones. 
% However, the scheme is struggling in the following situations. 
% First, given large-scale data sharing with massive keys, the simple scheme produces complex key management systems. 
% In addition, the access policies are empowered by the data owner in CP-ABE. Frequent updates to access policies require data owners to cumbersomely generate new ciphertext. PRE \cite{blaze1998divertible} can mitigate these problems by directly converting one key's ciphertext to another key's ciphertext through a proxy. The data owner can re-encrypt the data through the proxy when performing authorization conversion. The complex management problem of keys can be alleviated.


\textit{Data Usage:} As shown in Figure 
\ref{Fig::DataACRE} (II), the edge computing ecosystem has pervasive data analytics. In particular, data analytics exists in some edge servers, whose responsibility is to analyze raw data. For instance, as mentioned \ding{172}\ding{174} arrows, the collected raw data is to be used. Besides, data analytics also exists in some edge servers, which use some computation results shared from other servers for high-level analysis, as \ding{179} arrow indicates.
%, {\color{red}and in the cloud, which aggregates the global data for overall analytics.} 
Data owners could expect to learn how their outsourced data is used and control its usage (denoted as \textbf{RU1} \& \textbf{RU2} requirements).
However, the above access control models in data collection and storage would end their responsibility for protecting data after data access is granted. DUC could satisfy data sovereignty requirements because it enforces further flexible control by data usage restrictions. 
%In the edge computing ecosystem, it is challenging to keep data usage compliant with the data usage policy.




\textit{Securing Critical Access Control Data:} In summary, because the typical access control models mentioned in the above data lifecycles are not derived from edge computing natively, we should attempt to enforce them effectively in distributed edge computing to achieve low resource consumption and delay for access control, while ensuring flexibility and scalability. However, an access control system generally includes a wealth of sensitive access control data \cite{BlockchainforAC}.
For example, CapBAC includes authorization tokens, token registration, delegation, and revocation functions.
ABAC contains various attributes, attribute-based policies, and programs for enforcing policy. Some important access control data should be protected, e.g., sensitive tokens, private attributes, critical policies, and enforcement programs. 

%\textit{Blockchain for Secure Access Control.} 
%Blockchain can satisfy these data protection requirements. Because smart contracts can be coded distributedly to enforce access control and the security of enforcement results is guaranteed by the consensus mechanism, blockchain can be used as a trustable alternative for enforcing access control policies. 
Blockchain can be used to store important access control data because, as introduced in Section \ref{Sec::BlockchainTech}, it is a distributed database for storing data and the on-chain data is immutable. Moreover, accountability is natively provided because blockchain has immutability and traceability properties. 
Besides, smart contracts can be coded distributedly to enforce access control and the security of enforcement results is guaranteed by the consensus mechanism, and it can be used as a trustable alternative for enforcement programs. 
%Blockchain can simultaneously support the following requirements for accessing objects: decentralization, scalability, and trust.
As shown in Figure \ref{Fig::DataACRE} (III)(1)(2)(3), blockchain technology can enhance the access control mechanisms in data collection, storage, and usage, respectively. More precisely, the access control requirements for each data lifecycle can be achieved while safeguarding critical access control data.

Furthermore, the blockchain platform can also manage various access control enforcement. In particular, the blockchain platform can embody multiple access control functions, e.g., CapBAC for data collection, ABE for data storage, and DUC for data usage. 
%The blockchain-based versatile access control platform could offer comprehensive access control capabilities across multiple data lifecycles. 
That is, as shown in Figure \ref{Fig::DataACRE} (III)(4), a platform could satisfy all access control requirements (\textbf{RC1}\&\textbf{RC2}, \textbf{RS1}\&\textbf{RS2}, and \textbf{RU1}\&\textbf{RU2}) meanwhile access control data for multiple data lifecycles is uniformly managed.

\textit{Summary:} We have described the access control requirements by the common multiple lifecycles (including data collection, storage, and usage) while analyzing blockchain's role in protecting critical access control data. As shown in Table \ref{Table::ACReuqirementsTable}, we summarize the adopted typical access control models for satisfying the access control requirements in each data lifecycle and generalize the usage of blockchain to manage access control data. 
The contextual properties of CAAC can be integrated into ABAC, ABE, and DUC. In particular, the environmental properties of ABAC can use the contextual properties of CAAC to achieve access control; ABE can use them to encrypt/decrypt sensitive data; DUC can use them to control how to use data. Moreover, the role in RBAC can be regarded as an attribute of ABAC/ABE and a component of DUC.
The integration can facilitate the flexibility of access control. 
Finally, because consensus algorithms in blockchain possibly induce large latency, we should protect critical access control data with acceptable latency.
\textit{Note that, we do not present exhaustive access control models for each data lifecycle in edge computing due to the complexity.
The researcher or developer in the field can make systematical selections and innovations based on the
related access control techniques. This survey can prompt the development of access control techniques in edge computing under the intricacy of innovations in access control.
}

In the following sections, we will describe the recent solutions to use these typical access control models as base models for implementing access control in edge computing: 1) access control in data collection (Section \ref{Sec::ACInDataCollection}), 2) access control in data storage (Section \ref{Sec: ACInDataStorage}), 3) access control in data usage (Section \ref{Sec::ACInDataUsage}), and 4) blockchain-based access control platform (Section \ref{Sec::BBACP}).







==> Tex/Background.tex <==






% \subsection{Blockchain}

% \begin{figure}
% 	\begin{center}	\includegraphics[width=\columnwidth]{AllFigures/BlockchainArchitecture.pdf}
% 		\caption{Blockchain architecture}
% 		\label{Fig::DataACRE}
% 	\end{center}
% \end{figure}

% A blockchain system typically consists of 6 layers \cite{yuan2018blockchain}, namely the data layer, network layer, consensus layer, incentive layer, contract layer, and application layer. The data layer stores block data by database. The network layer is responsible for maintaining the connection and communication of the blockchain network. It ensures that different nodes can pass messages, exchange data, and synchronize the state of the blockchain. The consensus layer deals with the consistency between nodes, that is, to determine which transaction will be packaged into the next block. The consensus nodes of the blockchain are self-interested, and the maximization of revenue is the fundamental goal of its participation in data verification and bookkeeping. Therefore, an incentive compatibility mechanism should be designed to ensure that the goals of individual nodes are consistent with the overall goal of a safe and effective blockchain ecosystem. The contract layer encapsulates various types of script codes, algorithms, and complex smart contracts, and underpins the flexible programming and operation of blockchain systems. 
% At the application layer, various blockchain applications can be built.
% These applications leverage underlying blockchain technology to create secure, transparent, and tamper-resistant systems, enhancing trust, accountability, and efficiency across multiple industries and domains.


% The blockchain is a kind of distributed ledger technology. The committed transactions are recorded in the block. The linked block has the cryptographic hash summary of the content of the previous block. Blockchain is tamper-evident and tamper-resistant \cite{zheng2018blockchain}. The coded contract in a smart contract on a blockchain is deployed to and executed by blockchain nodes. And, smart contracts can satisfy the common contract items and the need for trusted intermediaries \cite{zheng2018blockchain}. The execution results are ensured to be correct due to the consensus mechanism in the blockchain.
% %so that the verification of calculation results is avoided in IoT devices. 
% Moreover,
% storing data in a distributed blockchain network reduces the risk of a single point of failure.

% Blockchain can be divided into permissionless and permissioned blockchains. Permissionless blockchain allows anyone to join, e.g., the popular public blockchain systems, bitcoin \cite{nakamoto2008bitcoin} and Ethereum \cite{wood2014ethereum}. Permissioned blockchain allows legal users of blockchain to participate, e.g., the consortium blockchain, Hyperledger Fabric \cite{androulaki2018hyperledger}.

\section{Typical access control models and Blockchain Technology}

\label{Sec::TraAccessControl}

\subsection{Typical access control models}
The access control model formally defines how subjects, objects, actions, conditions, and authorization policies are represented. And, the authorization policies regulate which object(s) can be accessed by which subject(s) with which action(s) under what condition(s). 
An access control mechanism is enforced according to an access control model and ensures that the objects can be controlled and used legally by reasonable access control. 


Many typical and popular access control models are available in academia and industry, such as,
Capability-Based Access Control (CapBAC) \cite{hernandez2013distributed}, Role-Based Access Control (RBAC) \cite{ferraiolo2001proposed}, Attribute-Based Access Control (ABAC) \cite{hu2013guide}, Data Usage Control (DUC) \cite{sandhu2003usage, park2004uconabc}, Group-Based Access Control (GBAC) \cite{GBAC}, Context-Aware Access Control (CAAC) \cite{toninelli2006semantic}, Risk-Aware Access Control (RAAC) \cite{atlam2020risk}, Relationship-Based Access Control (ReBAC) \cite{fong2011relationship}, and Trust-Based Access Control (TBAC) \cite{almenarez2005trustac, mahalle2013fuzzy}. To organize this survey, we classify RAAC, ReBAC, and TBAC into CAAC, and we will explain in the following. 

Access Control Lists (ACLs) \cite{grunbacher2003posix} are the most common access control, where the access right on resources is represented by a sequence of pairs $\langle$subject, operations$\rangle$. However, the list would become complex with the increment of subjects and resources.
To overcome the deficiency, RBAC \cite{ferraiolo2001proposed} introduces the role concept, which decouples the subjects and resources by assigning rights to the role(s) of subjects. Thus, RBAC reduces the efforts to manage access rights. However, in a large number of resources or cross-organization scenarios, the role explosion still needs lots of effort to be conquered. ABAC \cite{hu2013guide} uses properties of subjects, objects (resources), and environment to specify access rights, which exploits more components to manage access rights. This fashion could mitigate the role explosion problem but with the expense of more complex attributes components and access rules. However, the common problem of ACLs, RBAC, and ABAC is that they enforce access control by checking the union of all rights in a request.  
To avoid unnecessary traversal in the checking, CapBAC \cite{hernandez2013distributed} authorizes access rights by subject-oriented linked list,
a sequence of pairs $\langle$object, rights$\rangle$. CapBAC could achieve minimal privilege enforcement by checking the request-specified legal capability. Efficient capability revocations and updating can be easily enforced. 
However, CapBAC needs to issue capabilities for all subjects by cryptographic techniques. 


GBAC is a group-based model, where entities with the same permission requirements are assigned to the same group. Each group has specific access rights and attributes. Administrators can create groups of different levels as needed to achieve finer access control.
The inappropriate management of groups likely induces poor access control performance.

We can further incorporate context information in access control to enhance access permission management. 
In CAAC, access permissions are determined based on the combination of the subject, object, and other contextual information. CAAC can utilize this contextual information to adjust access permissions dynamically, thereby better meeting specific requirements and enhancing security. Contextual information may include basic ones, such as time, location, device status, network conditions, etc, and derived ones, such as trust, risk, relationship, etc. We mainly introduce the TBAC, RAAC, and ReBAC for this survey. 1) TBAC: In the era of pervasive computing resources and IoT devices, it is common that trust between entities cannot be established beforehand. TBAC focuses on enforcing access control by evaluating the trust level of the subject or object when trusted identities are not determined mutually. 2) RAAC:
In RAAC, the authorization of an access request depends 
%not only on the identity or role of the user but also 
on the risk factors associated with that request. These risk factors may include user behavior patterns, device security status, network security status, etc. The system dynamically adjusts access permissions based on these risk factors to provide appropriate resource access at different risk levels. 3) ReBAC:
ReBAC emphasizes the relationship between subjects in authorization decisions. The relationship can be diversified, such as superior-subordinate, cooperative, friendly, etc. Administrators can use the relationship to define access rights.


% With the development of information and communications technology, many access control models have been proposed and developed. 
% There are several typical and popular access control models, such as 
% %access control lists (ACLs) \cite{grunbacher2003posix}, 
% capability-based access control (CapBAC) \cite{hernandez2013distributed}, role-based access control (RBAC) \cite{ferraiolo2001proposed}, attribute-based access control (ABAC) \cite{hu2013guide}, data usage control (DUC \cite{sandhu2003usage, park2004uconabc}, group-based access control (GBAC) \cite{GBAC}, context-aware access control (CAAC) \cite{toninelli2006semantic}, risk-aware access control (RAAC) \cite{atlam2020risk}, relationship-based access control (ReBAC) \cite{fong2011relationship}, and trust-based access control (TBAC) \cite{almenarez2005trustac, mahalle2013fuzzy}. To organize our reviews, 
% we
% %refer to ABE as a special ABAC and
% classify RAAC, ReBAC, and TBAC into CAAC, and we will explain in the following. 

% \ding{172} \textbf{\textit{CapBAC:}} 
% %In access control matrix \cite{ACM}, This fashion possibly induces storage waste when many cells are null. 
% In traditional access control lists (ACLs),
% %stem from the access control matrix, where rows and columns represent subjects and objects respectively, and the cells describe rights. 
% %In ACLs, 
% an object-oriented linked list is linked with a sequence of pairs $\langle$subject, rights$\rangle$. 
% %The null cell is avoided. 
% The list must be traversed for enforcing ACLs, which induces unnecessary performance overhead.
% Compared with ACLs, the main idea in CapBAC is a subject-oriented link list. Each list heads with a subject concatenated by a sequence of pairs $\langle$object, rights$\rangle$. Without storing and checking all access control policies, CapBAC enables efficient enforcement for authorizing subjects to get resources. However, CapBAC requires additional token management based on cryptography.

% \ding{173}
% \textbf{\textit{RBAC: }}In RBAC, roles are the essential element for achieving access control. The mapping from subject to role(s) is accomplished by the administrator. The rights of objects are bounded by roles. RBAC takes advantage of roles for decoupling authorization with subjects. However, lots of effort is required to avoid role explosion.


% \ding{174}
% \textit{\textbf{ABAC: }}ABAC is an attribute-centric model. The attributes in ABAC can be characteristics of anything that may be defined, e.g., the roles of subjects. The attributes of subjects, objects, and environmental conditions are combined to control access to resources. ABAC is suitable for scenarios, where data protection is considered across different organizations. However, ABAC could induce complicated the problem of attribute management.  

The above access control models are non-cryptographic access control, which only controls data access according to access control policies. However, the data can be easily leaked if the access control is bypassed. With cryptography for access control, we can control data access according to access control policies while the protected data is encrypted \cite{huang2020attribute}.
The Attribute-Based Encryption (ABE) is a popular scheme in this kind of approach.
%\cite{huang2020attribute} can be viewed as a kind of ABAC. %We separately describe them for better presenting the recent efforts.
In an ABE-based system, data decryption is contingent upon the alignment of attributes. Specifically, both ciphertexts and users’ keys carry specific attributes. A user can only decrypt the ciphertext if the user’s attributes (or access policy) match the ciphertext’s access policy (or attributes). 
Key-Policy Attribute-Based Encryption (KP-ABE) combines access policy with key and encrypts data with attributes. Ciphertext-Policy Attributes-Based Encryption (CP-ABE) combines attributes with keys and encrypts data with access policy.  
%ABE is immune to collusion attack. 
ABE-based access control has mobility, i.e., each distributed data-hosting party can be a policy enforcement point because the ciphertext of data is combined with the access control. However, as asymmetric encryption technology, ABE requires the extra management of the ciphertext and keys and is generally used for small data volumes.

As shown in Figure \ref{Fig::ABEAndMAABE}, traditional ABE requires the authority to manage keys based on legal attributes. Data owners and data users only interact with the key intermediary. The abnormal key intermediary (e.g., disrupted legal attributes, DOS attack because of hacker intrusion) can affect the whole ABE system. Otherwise, multi-authority ABE (MA-ABE) depends on many related attribute authorities, where we can configure attributes used for encryption and decryption. For example, we can set that decryption can succeed with at least $d_{k}$ authorities providing secret keys for data users. As such, we can use the MA-ABE to manage attributes distributedly and resolve the key escrow problem. 

\begin{figure}
	\begin{center}
	\includegraphics[width=\columnwidth]{AllFigures/ABEAndMAABE.pdf}
		\caption{Attribute-based encryption (ABE) and multi-authority attribute-based
encryption (MA-ABE) \cite{huang2020attribute}.}
		\label{Fig::ABEAndMAABE}
	\end{center}
\end{figure} 


% In practice, access rights are usually changed with the development of applications. To re-encrypt a ciphertext from one key to another without decrypting the original ciphertext, Proxy Re-Encryption (PRE) is crucial to accommodate the variable access rights \cite{ateniese2009key, chow2010efficient}.
% PRE schemes can be unidirectional or bidirectional. In a unidirectional scheme, the data owner can delegate to a proxy that can re-encrypt the data for the data consumer key but cannot re-encrypt the data back for the original key. In a bidirectional scheme, the proxy not only re-encrypts data from one key to another but also re-encrypts it back for the original key. However, PRE schemes generally consume lots of resources due to re-encrypting ciphertext. 


The above models have a common drawback: they lose control after the data is granted access. DUC restricts data usage to enforce more flexible control after the data has been granted. For example, a party can use DUC to restrict data usage after it shares its data with another party. The restriction rules are specified by data owners who want to control how their data can be used. DUC can satisfy multiple data sovereignty requirements \cite{otto2022designing}. For example, the data usage scope controls that data must be used by trusted nodes or services; the data usage purpose controls that data must be used for specific usage purposes; the living time controls that data must be deleted immediately after data is used. However, DUC needs additional expenditure to accomplish these functions, such as purpose management and recognition. 


\subsection{Blockchain Technology}
\label{Sec::BlockchainTech}
The blockchain is a kind of distributed ledger technology \cite{dabbagh2021survey, zhang2021resource, zheng2018blockchain}. The committed transactions are recorded in the block. The linked block has the cryptographic hash summary of the content of the previous block, which enables the blockchain to be tamper-evident and tamper-resistant. Storing data in a distributed blockchain network reduces the risk of a single point of failure. The coded contract in a smart contract on a blockchain can be deployed to and executed by blockchain nodes. And, smart contracts can satisfy the common contract items and the need for trusted intermediaries. The execution results are ensured to be correct due to the consensus mechanism in blockchain so that the verification of calculation results can be avoided. 

Blockchain can be divided into permissionless and permissioned blockchains \cite{dabbagh2021survey}. Permissionless blockchain allows anyone to join, e.g., the popular public blockchain systems, bitcoin \cite{nakamoto2008bitcoin} and Ethereum \cite{wood2014ethereum}. Permissioned blockchain allows legal users of blockchain to participate, e.g., the consortium
blockchain, Hyperledger Fabric \cite{androulaki2018hyperledger}.

==> Tex/Discussions_on_Existing_Works.tex <==
\section{Challenges and Future Research Directions}
\label{Sec::Discussions}
% Based on the aforementioned recent work, this section discusses access control from the data collection, storage, and usage, to the blockchain.
% {\color{red}
% We envisage some future research directions towards high-performance, cooperated, integrated, versatile, hybrid, intelligent access control, etc., from the perspective of edge computing access control systems.}



Apart from the aforementioned issues, there remain challenges and new research directions in edge computing access control to be discussed, as follows.




\subsection{Machine learning-based access control in edge computing}

Traditional access controls commonly depend on predefined rules and require laborious maintenance and updates. With the widely distributed resources in edge computing, the demand for a more dynamic and efficient access control system is escalating. 
Machine learning can play an important role in satisfying the demand \cite{nobi2022towards}, where trained machine learning models constitute some blocks in access control systems to automate and reduce labor. Some studies use machine learning technology in their access control systems, e.g., \cite{atlam2021fuzzy, zheng2022adaptive, ghosh2021case}. 
We would discuss and envisage future research directions in the following aspects.

\begin{itemize}
    \item 
\textbf{Limited datasets:} 
A complete access control policy is the prerequisite for effective data protection.
The natural language documents for access control requirements are essential sources of access control policies \cite{narouei2018automatic}. Natural language processing technology is the common tool for extracting access control policies from those documents. It identifies and analyzes policy information described in human language, and converts this information into structured data that computers can comprehend and process.  
For example, Freisleben et al.\cite{ait2017abac} present an approach based on K-nearest neighbors algorithms for clustering ABAC policies, which can reduce the number of policy rules by evaluating similarity. Text2Policy \cite{xiao2012automated} classifies sentences into four access control modes. If a sentence matches, it extracts the subject, action, and object from the sentence by using the comments of the sentence. Text2Policy does not support contextual information extraction, nor does it support complex sentence patterns. To overcome the above defects, Narouei et al. \cite{narouei2018automatic} improve semantic role labeling and introduce domain-specific knowledge to greatly improve the performance of extracting implementable policies from natural language access control policy documents. The above work can support RBAC, ABAC, and Access Control Lists, but they do not support DUC. Hosseinzadeh et al. \cite{hosseinzadeh2020systematic} systematically propose a method to extract implementable policies from data usage requirement documents from the perspectives of data owners: policy declaration, policy transformation, and policy negotiation.

\textit{Limitation:} These studies facilitate the development of techniques for extracting access control policies from natural language documents. However, the explored datasets are mostly from conventional domains such as education and medicine. The lack of datasets from edge computing, especially in IoT, could impede the development of its access control technologies.
Besides, real-world access control policies generally involve sensitive data, which obstacles the development of datasets.  

\textit{Possible Solutions:} Policy generation can mitigate the limitation \cite{nobi2022machine}. The existing approaches to generating policy are problematic, e.g., random policy generation and manual policy writing. The datasets created using these methods are idealized, and do not fully capture the complex authorization scenarios in the real world. To generate simulated data with a similar distribution to any realistic data, 
we can explore pre-trained models (e.g., GPT4 \cite{achiam2023gpt}), such that the study of machine-based access control can reduce the reliance on real-world open-source datasets.
The following aspects should be considered: 1) access control models, 2) application domains, and 3) different neural networks for data simulation.
Different access control models have different organizations about access control information so the pre-trained models have different performances on different models. 
%For example, as the attributes is the core concept of ABAC, we can use conditional tabular generative adversarial networks. 
Many applications in IoT, e.g., the Internet of Vehicles and smart homes, have different data flow and business parties. Different application domains require different data simulations.
In large-scale access control scenarios, business parties can leverage pre-trained models to simulate data, test the access control functions overall beforehand, and monitor access control systems timely. Different neural networks require different computation power and could have different performances for various access control models and application scenarios. To make a cost-effective data simulation, business parties should select appropriate pre-trained models. 



% \textit{Optimization of access control policies:} Although there has been a lot of work on access control policy extraction, they still cannot satisfy the requirement of complete access control policies for data protection. We can use machine learning to further optimize access control policies. For example, Outchakoucht et al. \cite{outchakoucht2017dynamic} propose a reinforcement learning algorithm to achieve dynamic, optimized, and self-adjusting security policies. Karimi et al. \cite{karimi2021automatic} propose an ABAC policy mining method from access logs based on unsupervised learning. It can extract ABAC policies that contain positive and negative attributes, as well as positive and negative relationship filters. The paper also proposes rule pruning and policy optimization algorithms to improve the quality of mined policies and simplify their maintenance.
% Iyer et al. \cite{iyer2018mining} propose an algorithm for mining ABAC policies from authorization logs. It can extract positive authorization rules and negative authorization rules from given access control information.
%跨组织或者联盟优化


% \textit{Transformation of access control system:} Actively learning new access control policies from traditional access control systems can significantly reduce the cost of directly constructing new access control policies, which can be achieved by introducing machine learning models. For example, Bui et al. \cite{bui2020decision} propose a decision tree-based DTRM algorithm for mining ReBAC policies from access control lists and information about entities. Bui et al. \cite{bui2020learning} propose an algorithm based on learning multi-way decision trees. When some attribute values of entities are unknown, it can still efficiently mine ABAC and ReBAC policies from access control lists and incomplete information about entities.
%{\CheckC Bui et al. \cite{bui2017mining} propose an algorithm for mining ReBAC policies from access control lists and attribute data represented as an object model, which incorporates a greedy algorithm.}
%% 跨组织或者联盟之间的联合模型升级，研究一下边缘智能中的模型迁移

\item

\textbf{Federated learning:} Different business organizations in the edge computing ecosystem would form alliances based on business interests. The aforementioned studies in data lifecycles can be used intra-alliance, in which data owners and consumers cooperate to exert IoT-generated data. Due to data owners' limited data protection ability, their access control policies may be incomplete. These data owners can use the access control policies of other data owners to enhance their access control policies, such as adding missed access control policies or updating inferior access control policies. For example, Abu Jabal et al. \cite{abu2023flap} propose FLAP, a federal learning framework for ABAC. It allows data owners to learn ABAC policies from each other, ensuring that each party generates accurate policies. Moreover, FLAP takes into account policy conflicts and privacy concerns. To solve the problem of insufficient access control policies in a single smart home IoT context, Yu et al. \cite{yu2020learning} propose the federal multi-task learning framework LoFTI for several federated smart homes. The framework ensures the privacy of the access control policy in a smart home, enhances its context-based access control policy, and realizes the personalization of the smart home policy. Federated learning could be feasible in the cross-domain optimization of access control policies. However, they have limited consideration of the complex data lifecycles in edge computing. Multi-data lifecycles indicate access control policies of multiple access control models. An interesting research direction is to optimize each data owner's access control policies of multiple access control models, meanwhile without privacy leaking among data owners. A possible solution could be versatile federated learning, targeting a multi-access control federated model, which allows data owners to enhance access control policy with less consideration of the access control models.

\item
\textbf{Adversarial attacks:} Although machine learning-based access control systems have the potential for enhancing data security in largely distributed edge computing, the deployment of such systems can be hampered by the vulnerability of machine learning models to adversarial attacks. These attacks exploit weaknesses in machine learning algorithms to violate the system's access control policies to gain unauthorized access. 
For example, Nobi et al. \cite{nobi2022adversarial} propose that adversarial attacks can be reduced to a certain extent by utilizing specific constraints on access control. We would further explore solutions for implementing machine learning-based access control and mitigating various attacks within the edge computing ecosystem. These solutions should consider the characteristics and features of access control in edge computing, such as various models and large scale. 

% \item 
% Various data usage scenarios have complicated data usage relationships. 
% Generally, purpose-based schemes rigidly designate static purpose(s) for data usage. 
% We can exploit the shared dynamic graph of data usage purposes to determine which usage purpose is legal. 
% As a result, purpose-based schemes adapt to the complicated data usage relationships in edge computing.


\end{itemize}





\subsection{Hybrid access control}

Hybrid access control technology can improve access control performance by combining the advantages of different access control mechanisms \cite{pal2021protocol}. In edge computing access control, the introduced models in Section \ref{Sec::TraAccessControl}, e.g., CapABC, ABE, and DUC, are a set of data security techniques.  As shown in Figure \ref{Fig::HybridAccessControl}, we can combine these models' components to enhance the performance of access control in edge computing.
For example, to satisfy the low-latency requirements and secure access control systems for the Industrial Internet-of-Things (IIoTs). DHACS \cite{saha2021dhacs} combines these elements: role, context, and organization regulation. The functions of access control are encoded in smart contracts. The operational transactions are recorded on the blockchain. The efficiency of access control management is improved by about 30\%. DHACS is the first attempt to use a decentralized blockchain with smart contracts for hybrid access control in IIoTs. 
Because services involve data analytics, it is reasonable to introduce appropriate components of DUC into CapBAC to optimize access control performance further. The components of purpose-based schemes can be applied to ABE-based access control, which could further restrict data usage in advance and reduce the computing cost of decryption by purpose. 
%To mitigate privacy leaks, attacks, and structural security in smart homes, Zhang et al. \cite{zhang2021blockchain} design an access control scheme in the smart home environment. In particular, the hybrid access control model supports dynamic ABAC and static access control matrix. Smart contracts are utilized to execute access control policies. The access requests are recorded on a blockchain. 

\begin{figure}
	\begin{center}
	\includegraphics[scale = 1.2]{AllFigures/Hybridaccesscontrol.pdf}
		\caption{Hybrid access control.}
		\label{Fig::HybridAccessControl}
	\end{center}
 \vspace{-0.2cm}
\end{figure} 

%In terms of data usage control, purpose-based and hardware-assisted usage control could be integrated to enhance the privacy of purpose. 

Hybrid schemes' effectiveness, efficiency, and flexibility can be researched for high-performance edge computing access control under pervasive data analytics.
For example, the method to make a more flexible CapBAC should be inspected when CapBAC is combined with DUC. The method to implement efficient decryption/encryption could be investigated when the purpose attribute is integrated into the ABE scheme. 

Finally, while hybrid access control can improve performance, privacy issues in hybrid models should be investigated because hybrid means that some cases involve organization-across attributes.




% Some challenges need to be conquered. 
% 1) Complex data flow will produce a variety of application scenarios, resulting in a very complex data lifecycle, and it is difficult to exhaust all application scenarios in advance.
% Existing research work fails to design versatile access control technology from the perspective of the data lifecycle. 
% 2) In an edge computing ecosystem, generating access control data is decentralized, and centralized data management is easy to cause system bottlenecks. 
% Although some efforts try to achieve decentralized management of access control data through blockchain, they tend to chain all relevant access control data by default, failing to consider the ease of data on the chain and off the chain. 
% This ease of use is crucial for the widespread use of blockchain, as blockchain users generally need to make a trade-off between the cost of using blockchain (e.g., the more data on the chain, the higher the cost \cite{international2018new}) and data security. 
% 3) The versatile access control system should meet the different latency and throughput requirements for diversified applications. 
% The latency and throughput of an access control system are related to access control functions and access control data management. 
% The existing research work has not systematically optimized the performance of access control systems from the perspective of access control function and access control data management.



% Moreover, the on-chain data has different features. 
% 1) Data update frequency is different. 
% For example, the registration of capability in CapBAC generally does not happen more frequently than the generation of data usage logs. 
% 2) The data type is different. 
% For example, the access policy may be expressed in various formats; log data and token data have different formats. 
% In essence, blockchain is a database. 
% It is straightforward that the strategy ``one kind of data feature has one blockchain'' is convenient for data management. 
% However, this strategy wastes resources (e.g., storage) for access control systems.
% We should find the trade-off between the number of used blockchains and the performance of access control. 
% To integrate various data for a unified blockchain, we should consider all the data features for saving storage space and keep the performance of the blockchain satisfying access control systems in edge computing.   


\subsection{Powerful access control technology testbed}

Some testbeds in the mentioned studies use simulation tools to verify their ideas. Some deploy complex real end-edge-cloud platforms, which enable the tests to be closer to real production scenarios. 
The new paradigm, i.e., edge computing \cite{EssentialsofEC}, has complex network topology (e.g., LAN, MAN, and WAN) and heterogeneous network devices (e.g., Cisco or Huawei switch). Meanwhile, IoT devices and edge nodes are heterogeneous with different computing, storage, and communication capabilities. Except for the sophisticated hardware conditions, heterogeneous IoT and network protocols coexist. For example, MQTT and XMPP are usually used to collect IoT-derived data in a certain security domain. WiFi and 5G enable devices to connect with and communicate in networks. 
Because this physical ecosystem has enormous economic expenditures and complex maintenance, it is difficult to achieve flexible and extendable tests for research and real production scenarios. 
%The edge computing access control testbed is not flexible enough and easy to use. 


To tackle these challenges, many open-source simulation tools for edge computing are developing \cite{mahmud2022ifogsim2, nandan2019iotsim, sonmez2018edgecloudsim}, which prompts the development of edge computing technology.  
They can simulate common infrastructures, including networks, mobile devices, edge data centers, microservices, edge orchestrators, edge clusters, and central cloud. Moreover, they support various computing loads, different data distributions, and access to real data.




These simulation systems do not consider the simulation of access control currently natively. However, they support powerful module customization and extension. These existing simulation systems can be extended to support access control simulation.
%, while access control, as a fundamental security technology, should deserve a thorough verification of its functions. 
To achieve this simulation in an edge computing ecosystem, similar to supporting various network protocols, these simulation systems should flexibly integrate heterogeneous access control models/protocols. For example, the attribute authorities and context information should be allowed according to the user's configuration in the simulation system.
It is not advisable to embed rigid access control models into simulation systems according to real experiences about applications, because the applications in edge computing are various and could be changed frequently. To integrate different access control models flexibly, we need a universal library for various model modules, each of which acts as a basic building block for constructing a functional model template. 
In addition, real data should be flexibly and advisably injected for the corresponding function verification in the light of real-world situations. 
Because access control would run on enormous data in real situations, capturing all real data in a simulation system is impractical.
The trade-off between the amount of ingested data and verification accuracy should be researched, especially considering diversified data categories in edge computing. 
Finally, the high usability of the simulation system would be an important problem to be solved, so that the system users can build the target access control system efficiently. As such, researchers or technicians can focus on verifying their ideas for implementing access control functions. 

%for stimulating the innovation of access control in edge computing.

% It is not advisable to embed rigid access control models into simulation systems according to real experiences about applications, because the applications in edge computing are various and could be changed frequently. To integrate different access control models flexibly, we need a universal library for various model modules, each of which acts as a basic building block for constructing a functional model template. 

% Because access control would run on enormous data in real situations, capturing all real data in a simulation system is impractical.
% %To accomplish function verification with real data, we should consider lightweight data ingestion while keeping the effectiveness of verification. 
% The trade-off between the amount of ingested data and verification accuracy should be researched, especially considering diversified data categories in edge computing. 

% The high usability of the access control simulation system mainly means that the system users can build the target access control system efficiently. As such, researchers or technicians can focus on verifying their ideas for implementing access control functions.
% A possible solution is to construct a simulation system by automatic or semi-automatic tools.
%by artificial intelligence. %We should train the artificial intelligence system with appropriate data. The functional description of access control may be the data because different applications likely expect different access control functions. Data classes may be the data because different access control functions are likely used on different categories of data. 
%Finally, the AI system should be interactive, where human language can be used to describe a simulation system, and a corresponding system is generated by AI.


% \subsection{Build the overall attributes library}

% Access control technologies exist widely in edge computing.
% In these technologies, the attributes derive from entities in the real world.
% To generate attributes set in a specific application, we collect and design attributes.
% However, with the development of applications in edge computing, highly personalized applications are developing \cite{kubiak2022possible, hartmann2022edge, hui2021secure, RealWorldUseCase} and new access control requirements possibly arise. Thus, the corresponding highly personalized access control mechanisms are expected. 

 
% For example, in connected and autonomous vehicles, the natural attributes of cars and attributes in the driving habits of drivers can be used by car owners to set what driving habits can only be collected and analyzed by the insurance company serving the car. 
% When combining the connected and autonomous vehicles scenario and health scenario, we should combine the attribute sets from both scenarios, such that flexible and rich access policies can be defined, especially in personal applications. 
% For example, data owners can set the regulation: some health data cannot be collected, but some data can be collected, for certain hospitals/institutes when their cars are used from 8:00 to 12:00. 


% The ample attributes are the fundamental facility for achieving the personalization. 
% The isolated attributes set in the legacy access control systems may be combined to achieve new access control functions. 
% In addition, applications could identify the special attributes used in their access control system. 
% As shown in Figure \ref{Fig::attributeset}, we can combine each attribute set according to application scenarios, however, the combination shows intricate connections, which challenges the management of attributes in pervasive edge computing access control. 
% If there is a universal attribute set containing enough common attributes, the attribute set construction complies with the rule of dependency inversion, which unburdens the pressure of attribute management. 
% Moreover, some specific attributes for new applications could be shared for future applications. 
% As a result, a convenient and management-friendly attributes ecosystem for edge computing is generated.   


% \begin{figure}
% 	\begin{center}
% 	\includegraphics[width=\columnwidth]{AllFigures/universalattributes}
% 		\caption{In edge computing, coupled attribute sets are changed into decoupled ones for flexibly achieving high personalized access control mechanisms}
% 		\label{Fig::attributeset}
% 	\end{center}
% \end{figure}


% Although universal attributes set can facilitate access control, the comprehensive attributes in edge computing challenge data privacy. 
% Many visual attributes from computer vision at the edge can be learned, e.g., age, height, muscle, color, and posture attributes.
% Social attributes from common social information can be ingested, e.g., ID card age and family relationship.
% Health attributes can be obtained from the sensed information for wearable devices, e.g., heartbeats and driving under the influence. 
% Universal attributes set must be protected appropriately, otherwise, personal data possibly be leaked.




% {\CheckC This section envisages future research directions from the following seven aspects: high-performance CapBAC in a high-dynamic environment, high-performance data cryptography for access control, cooperated data usage control, integrated blockchains for access control in edge computing, access control technology testbed for edge computing, hybrid access control, and overall attributes library.}


==> Tex/Introduction.tex <==
\section{Introduction}

In the Internet of Things (IoT) era, massive devices generate enormous data, which is collected, stored, and analyzed for fueling many contemporary applications, such as smart homes and smart cities \cite{gomez2019internet}. 
As the pivotal infrastructure, cloud computing is used to harness these data. 
However, the latency, mainly induced by the geographical distance between data sources and cloud centers, would be unacceptable for some applications, such as virtual realization and connected autonomous vehicles.   
To address these challenges, edge computing acts as a synergistic technique to cloud computing, so that computing resources are situated closer to data sources and large raw IoT data is processed locally in edge nodes. Subsequently, the processed data could be transmitted to the cloud for advanced analysis \cite{chen2019deep}. 
Therefore, edge computing can help alleviate network burdens for the cloud, support latency-sensitive applications, and simultaneously enhance data security \cite{shi2016edge}. 

Access control for data security is always accompanied by the development of new technology \cite{ferrari2010access, shi2016edge}, and edge computing is no exception. Access control ensures that only authorized users and devices can access sensitive data stored at the edge nodes. The number of security incidents caused by internal users or system errors at the edge nodes can be reduced through stringent access control. Access control helps enterprises ensure that their edge computing practices comply with regulations such as GDPR \cite{custers2019eu}.

Access control is commonly developed based on many typical and popular access control models, such as Capability-Based Access Control (CapBAC) \cite{hernandez2013distributed}, Role-Based Access Control (RBAC) \cite{ferraiolo2001proposed}, Attribute-Based Access Control (ABAC) \cite{hu2013guide}, Data Usage Control (DUC) \cite{sandhu2003usage, park2004uconabc}, Group-Based Access Control (GBAC) \cite{GBAC}, Context-Aware Access Control (CAAC) \cite{toninelli2006semantic}, Risk-Aware Access Control (RAAC) \cite{atlam2020risk}, Relationship-Based Access Control (ReBAC) \cite{fong2011relationship}, and Trust-Based Access Control (TBAC) \cite{almenarez2005trustac, mahalle2013fuzzy}. In this survey, CAAC includes basic CAAC and derived CAAC. Basic CAAC considers raw context data, e.g., location. Derived CAAC considers trust, risk, and relationship (corresponding to TBAC, RAAC, and ReBAC respectively), which should be computed based on raw data. Besides, there are also typical cryptography-based access controls, such as Attribute-Based Encryption (ABE). We will detail these access control models in Section \ref{Sec::TraAccessControl}. 

To enhance data protection in edge computing, numerous studies have been dedicated to exploring these access control models to realize their potential improvements/implementations in edge computing scenarios. 
%Although edge computing offers numerous benefits,
These studies confront several significant challenges of access control, which edge computing introduces. Firstly, a wide range of IoT devices in edge computing often operate with limited resources like storage, computational power, and communication capabilities. The resource-constrained environments pose challenges for effectively implementing the access control mechanisms that typically require many resources. Secondly, the latency in edge computing results from various factors like task offloading, communication duration, computational expenses, and security measure-induced overheads. To preserve its low latency advantage, the implementation of access control systems must not significantly extend these delays.
%The time for enforcing access control should remain within reasonable bounds to ensure that the low latency benefit is not negated by the delay caused by the implementation of access control systems.
Thirdly, the mobile nature of data producers and consumers in edge computing scenarios necessitates flexibility in access control mechanisms to accommodate this dynamism. 
Lastly, the widespread geographical distribution of edge nodes challenges the scalability of centralized access control systems and complicates trust management in such a decentralized environment.


It is important to summarize these studies for the development of access control technologies in edge computing. 
Several surveys on this topic have been published, usually from a different perspective.
%lack systematic research according to data lifecycles.
Kayes et al. \cite{kayes2020survey} make the review for CAAC. They systematically review the basic contextual conditions, e.g., temporal, location, and spatial, and the derived ones, e.g., relationship. And, they introduce how CAAC works with RBAC and ABAC for adapting to the dynamic environment in edge computing.
Zhang et al. \cite{zhang2018survey} present CapBAC, ABAC, ABE, RBAC, and DUC in edge computing. However, they do not cover GBAC and CAAC. 
Alnefaie et al. \cite{alnefaie2021survey} survey the CapBAC, ABAC, DUC, and RBAC, meanwhile, introducing CAAC (basic and TBAC), but without ABE, GBAC, RAAC, and ReBAC. Rasori et al. \cite{ABESurvey} focus on reviewing suitable ABE for IoT, which assumes that the edge servers are untrusted. To spur the development of DUC, Akaichi et al. \cite{akaichi2022usage} review various DUC proposals for their specification, enforcement, and robustness.
%However, this work does not provide PRE, GBAC, RAAC, and blockchain-based schemes of ABE, PRE, and DUC. 

While the aforementioned studies make their reviews with different access control models, they do not consider blockchain-based access control, which is an emerging and widely adopted novel access control technology.
% Ragothaman et al. \cite{ragothaman2023access} survey CapBAC, ABAC, RBAC DUC, ReBAC, and blockchain-based access control.
Pal et al. \cite{pal2022blockchain} mainly present the studies to use blockchain for enhancing CapBAC, RBAC, TBAC, and ABAC in edge computing. 
Riabi et al. \cite{riabi2019survey} present blockchain-based access control for improving ABAC, RBAC, and CapBAC.
%Mahamuni et al. \cite{mahamuni2023blockchain} focus on the review of PRE and its blockchain-based scheme.
Khan et al. \cite{khan2022authorization} classify the existing authorization mechanisms, weaknesses, and loopholes. 
The CapBAC, ABAC, ABE, TBAC, and their corresponding blockchain-based schemes are involved. 
Dram{\'e}-Maign{\'e} et al. \cite{drame2021centralized} survey the access control solutions from the perspectives of architectures, e.g., centralized, hierarchical, federated, and distributed. The CapABC, ABAC, ABE, RBAC, CAAC, and general blockchain-based access control are analyzed in these architectures. 


%Qiu et al. \cite{qiu2020survey} present CapBAC, BCapBAC, ABE, DUC, CAAC, TBAC, and ReBAC in IoT systems. 

Moreover, 
Ravidas et al. \cite{ravidas2019access} divide the requirements of access control systems into three categories according to policy lifecycles, i.e., policy specification, policy management, and policy evaluation\&enforcement. This survey analyzes CapBAC, ABAC, DUC, RBAC, and CAAC according to the above classifications.


However, the aforementioned studies do not consider the reviews from the perspective of multiple data lifecycles. In edge computing, data security encompasses multiple stages including data collection, storage, usage, etc. A comprehensive review of access control techniques across multiple data lifecycles can facilitate the holistic technique advancement.
Khalid et al. \cite{khalid2021survey} survey on secure data storage and retrieval in edge computing. 
It involves ABE and TBAC and discusses the corresponding management issues.
Liu et al. \cite{liu2019survey} conduct a comprehensive review on secure outsourced data analytics in edge computing. 
Secure data collection covers authentication mechanisms and trust management mechanisms. 
Secure data processing relies on the following techniques: homomorphic encryption, differential privacy, pseudonym technology, etc. 
Data processing generates computational results, which could be stored and kept protected. 
Secure data storage usually leverages access control mechanisms (e.g., ABE and RBAC) and searchable encryption (including symmetric and asymmetric methods). However, this work does not involve CapBAC, DUC, GBAC, and the related blockchain-based schemes. 


%To describe these surveys and make clear comparisons, we list the abbreviations in Table \ref{Table: Acronyms}. 

% \subsection{Opportunities}
% These challenges stimulate the development of access control technologies in edge computing. The key areas are listed as follows.

% 1) \textbf{Resource-Optimized Access Control Algorithms}: Confronted with the challenge of limited resources on IoT devices, we have a prime opportunity to innovate with more streamlined and resource-conserving access control mechanisms. 
% %Such mechanisms are envisaged to lean on computational and storage demands while upholding stringent security standards. 
% % For instance, exploring capability-based access control (CBAC) models adapted for edge environments offers a compelling alternative. In CBAC systems, devices or users are granted capabilities or tokens that explicitly define their access rights to resources. This approach can be optimized for IoT contexts by integrating lightweight cryptographic techniques and efficient token management strategies. These tokens can be dynamically issued and adjusted based on contextual information such as the device's current operational state, its network environment, and predefined access policies. 
% %By utilizing such a model, it's feasible to 
% Such mechanisms are envisaged to achieve granular and flexible access control that scales efficiently across the diverse and distributed nature of IoT devices, all the while minimizing the resource footprint on these constrained devices.

% 2) \textbf{Low-Latency Access Control Systems:} In response to latency issues, researchers and developers can explore new access control architectures and protocols specifically designed to reduce enforcement time and minimize the latency introduced by security measures. Developing distributed access control systems that leverage edge computing capabilities for rapid local enforcement can reduce dependence on central servers and communication latency.

% 3) \textbf{Dynamic and Adaptive Access Control Strategy:} The mobility of data producers and consumers presents an opportunity for developing access control mechanisms that can adapt to changing environments and user needs. These systems could adjust access permissions in real time to accommodate changes in user location, network conditions, or device status, providing more flexible and personalized security.

% 4) \textbf{Distributed and Decentralized Access Control Models:} The challenge of managing the widespread geographical distribution of edge nodes calls for decentralized access control models. Leveraging technologies such as blockchain \cite{yuan2018blockchain}, these models can enhance the scalability and resilience of access control systems, increase data transparency, and boost user trust. Moreover, such models can simplify trust management and permission verification processes, ensuring the effective enforcement of security policies in a distributed environment. 

%For example, context-aware access control is explored for exploiting abundant context information to accomplish flexible access control. Capability-based access control is designed to collect data from resource-limited IoT devices efficiently. 
% Attribute-based encryption and proxy re-encryption are further studied to facilitate data storage and sharing. 
% %Effective and efficient data usage control is explored to facilitate data protection after data is granted access.
% Blockchain-based access control can simultaneously support the decentralization, scalability, and trust for accessing objects.

% \begin{table*}[]
% \centering
%  		\setlength{\abovecaptionskip}{-0cm}
% 		\setlength{\belowcaptionskip}{-0cm}
% \caption{Comparison of our survey to other related works}
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \label{Table::ComparisonofSurvey}
% Ref & CapBAC & BCapBAC &ABE & BABE & PRE & BPRE & DUC & BDUC & CAAC & TBAC & GBAC & RAAC & ReBAC \\ \hline
%  \cite{kayes2020survey}           &   -     &    -       &   -  & -  &- & -    & -    &  -         & \checked  & - & -&- & \checked     \\ \hline
% \cite{zhang2018survey} & \checked & - &  \checked & - & \checked &  - & \checked  & -   &  -   & -   & - & - & -        \\ \hline
% \cite{alnefaie2021survey}           &  \checked  & -  &  -   & - &- & -  & \checked & -          &  \checked  &  \checked   &- &- & -        \\ \hline
% \cite{ravidas2019access}          &  \checked      &  -         &  -   & - & - & -    &  \checked  &  -         &  \checked  &   \checked    &- &- & -\\ \hline
% \cite{pal2022blockchain} & - & \checked  & -   &   \checked & - &  -     &  -   &  -         &   \checked     &       \checked   &- &- &-   \\ \hline
% \cite{khalid2021survey} &  -      &  -   & \checked & -   & \checked &  -  &  -   & -   &   -   & \checked  &- & -& -\\ \hline
% \cite{ragothaman2023access}           &  \checked   &  -   &  - & - &- & -& \checked  &  -         & \checked  &  \checked   & -& \checked & \checked        \\ \hline
% \cite{ABESurvey}  &   -     &   -        &   \checked  & -   & - & -       &  -   &-           &   -            & -      &- &- &-      \\ \hline
% \cite{riabi2019survey}
%  & \checked &  \checked  & -  &  -  & - &   -    &  -   &    -       &   -     &  - & -& -& -\\ \hline
% \cite{mahamuni2023blockchain}  & - & - &  -  &  -  & \checked & \checked  &  -   &-           & -          & -  & -& -&- \\ \hline
%  \cite{akaichi2022usage}           &  -      &  -         & -    & -  &- &- &-   \checked  & -    & -  &  -       & -& -&-    \\ \hline
%  \cite{drame2021centralized}           &  \checked        &  \checked  &  \checked   & -  & -& - &  \checked  & -    &  \checked  &  \checked        & \checked  &- & \checked    \\ \hline
%  \cite{liu2019survey}  &  -      &   -        &   \checked  & -   & \checked & -      & -    &   -        &        \checked   &  \checked  &- &- &- \\ \hline
% \cite{qiu2020survey}           &   \checked & \checked & \checked & - & -& -  & \checked &    -       &  \checked  &  \checked & -& -& \checked \\ \hline
%  \cite{khan2022authorization}           &   \checked & \checked & \checked & \checked & -& -  &- &  -         &  \checked  &  \checked &- & -&- \\ \hline
% Our & \checked & \checked & \checked & \checked & \checked & \checked & \checked  & \checked  & \checked & \checked        & \checked & \checked  & \checked    \\ \hline
 
% \end{tabular}
% \vspace{-0.1cm}
% \end{table*}

% \begin{table*}[]
% \centering
%  		\setlength{\abovecaptionskip}{-0cm}
% 		\setlength{\belowcaptionskip}{-0cm}
% \caption{Comparison of our survey to other related works}
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \label{Table::ComparisonofSurvey}
% Ref & CapBAC & B1 & ABAC & B2 & ABE & B3 & PRE & B4 & DUC & B5 & RBAC & B6 & GBAC & CAAC[Basic, TBAC, RAAC, ReBAC] \\ \hline
%  \cite{kayes2020survey}           &   -     &    -  &  \checked &      &   -  & -  &- & -    & -    &-&\checked & &-& [\checked,-,-,\checked]     \\ \hline
% \cite{zhang2018survey} & \checked & - & \checked & &  \checked & - & \checked &  - & \checked  & -   & \checked &  &-&  [-,-,-,-]        \\ \hline
% \cite{alnefaie2021survey}           &  \checked  & - & \checked & &  -   & - &- & -  & \checked & - & \checked  & & - &  [\checked,\checked,-,-]        \\ \hline
% \cite{ravidas2019access}     &  \checked &  -  &  \checked & &  -   & - & - & -    &  \checked  &  -  & \checked & & -&  [\checked,\checked,-,-]\\ \hline
% \cite{pal2022blockchain} & \checked & \checked  & \checked  & \checked & \checked   &   \checked & - &  -     &  -   &  -         &   \checked  & \checked &- &    [\checked,\checked,-,-]   \\ \hline
% \cite{khalid2021survey} &  -      &  -  &  & & \checked & -   & \checked &  -  &  -   & -   &   -   & & & [\checked,-,-,-]\\ \hline
% \cite{ragothaman2023access}           &  \checked   &  -  & & &  - & - &- & -& \checked  &  -         & \checked & &  &  [\checked,-,\checked,\checked]        \\ \hline
% \cite{ABESurvey}  &   -     &   -   &     & &   \checked  & -   & - & -       &  -   &-          & & &   -            & [-,-,-,-]      \\ \hline
% \cite{riabi2019survey}
%  & \checked &  \checked & & & -  &  -  & - &   -    &  -   &    -    &  & &   -     &  [-,-,-,-]\\ \hline
% \cite{mahamuni2023blockchain}  & - & - &  -  & &  -  & \checked & \checked  &  -   &-           & & -       & &  & [-,-,-,-] \\ \hline
%  \cite{akaichi2022usage}           &  -      &  -  &      & & -    & -  &- &- &-   \checked  & -   & & & -  &  [-,-,-,-]    \\ \hline
%  \cite{drame2021centralized}           &  \checked        &  \checked  & & &  \checked   & -  & -& - &  \checked  & -    & & &  \checked  &  [\checked,\checked,-,\checked]    \\ \hline
%  \cite{liu2019survey}  &  -      &   -     &   & &   \checked  & -   & \checked & -      & -    &   -      & & &        \checked   &  [\checked,-,-,-] \\ \hline
% \cite{qiu2020survey}           &   \checked & \checked & & & \checked & - & -& -  & \checked &    -      & & &  \checked  &  [\checked,-,-,\checked] \\ \hline
%  \cite{khan2022authorization}           &   \checked & \checked & & & \checked & \checked & -& -  &- &  -        & & &  \checked  &  [\checked,-,-,-] \\ \hline
% Our & \checked & \checked & & & \checked & \checked & \checked & \checked & \checked  & \checked  & & & \checked & [\checked,\checked,\checked,\checked]    \\ \hline
 
% \end{tabular}
% \vspace{-0.1cm}
% \begin{tablenotes}
%      \item[1] -: It is not mentioned in this work.
%      \item[2] CAAC definitions at Section. 
% \end{tablenotes}
% \end{table*}

%\subsection{Traditional Access Control: Solutions and Limitations}
%\label{Sec::AC}
%Access control is the fundamental technology for data management systems. 





% \begin{table}[]
% \centering
% \caption{List of models and their abbreviations}
% %\resizebox{\linewidth}{!}{
% \begin{tabular}{|l|l|}
% \hline
% \label{Table: Acronyms}
% \textbf{Acronyms} & \textbf{Models} \\ \hline
% CapBAC & Capability-based Access Control              \\ \hline
% %B1 & Blockchain-Based Capability-based Access Control              \\ \hline
% ABAC   & Attribute-Based Access Control               \\ \hline
% %B2     & Blockchain-Based Attribute-Based Access Control \\ \hline
% ABE    & Attribute-Based Encryption                          \\ \hline
% %B3 & Blockchain-Based Attribute-Based Encryption              \\ \hline
% PRE    & Proxy Re-encryption                          \\ \hline
% %B4    & Blockchain-Based Proxy Re-encryption     \\ \hline
% DUC  & Data Usage Control                          \\ \hline
% %B5 & Blockchain-Based Data Usage Control              \\ \hline
% RBAC   & Role-Based Access Control                    \\ \hline
% %B6       & Blockchain-Based Role-Based Access Control  \\ \hline
% GBAC   & Group-Based Access Control                 \\ \hline
% CAAC   & Context-Aware Access Control  \\ \hline
% TBAC & Trust-Based Access Control         \\  \hline
% RAAC & Risk-Aware Access Control    \\   \hline
% ReBAC & Relationship-Based Access Control                 \\ \hline
% %CP-ABE & Ciphertext-Policy Attribute-Based Encryption \\ \hline
% %KP-ABE & Key-Policy Attribute-Based Encryption \\ \hline
% %ACLs    & Access Control Lists                         \\ \hline
% %VACP    & Versatile Access Control Platform            \\ \hline
% \end{tabular}

% \begin{tablenotes}
%      \item[1] Note: In this article, CAAC includes basic CAAC, TBAC, RAAC, and ReBAC. Basic CAAC considers raw context data, e.g., location. Derived CAAC considers trust, risk, relationship, etc., which should be computed based on raw data.
% \end{tablenotes}

% \vspace{-0.1cm}
% \end{table}




Although there are surveys on edge computing access control according to different data lifecycles, they do not systematically consider those typical access control models in the third paragraph and lack the corresponding blockchain schemes for each model. This motivates us to have a more comprehensive and systematic survey with the following contributions: 
% 尽管有些survey站在数据生命周期的角度进行了survey, 但是。。。models 覆盖不全，不能系统的展示blockhcain在访问控制中的作用。。。
% Our proposed survey is focused on reviewing access control in multiple data lifecycles. 
% Our contributions are summarized as follows: 

\begin{itemize}
    \item 
% Based on the recent surveys of edge computing access control, 
According to the architecture of edge computing, we analyze the access control requirements from data collection, data storage, and data usage, and the role of blockchain in protecting critical access control data in these data lifecycles. In particular, we show how to use/enhance the CapBAC, ABAC, ABE, DUC, RBAC, GBAC, CAAC (basic, TBAC, RAAC, and ReBAC), and blockchain from the perspective of these data lifecycles.

 \item 
     Following the systematic requirements analysis, we present and discuss the recent studies on access control techniques in edge computing, and provide the lessons learned from the involved studies.

\item According to the discussions about the recent research studies, we discuss challenges and research directions of access control in edge computing. 
    
\end{itemize}

For the reader's convenience, we classify the related studies to be discussed in this survey in Figure \ref{Fig::Classification}.
Our classification does not cover every aspect of access control due to the complexity of access control in edge computing. However, this survey can complement existing surveys, which can help readers understand edge computing access control systematically. Further, the researcher or developer in the field can make systematical selections and innovations based on the related access control techniques. 
This survey can prompt the development of access control techniques in edge computing under the intricacy of innovations in access control.

\begin{figure}
	\begin{center}
	\includegraphics[width=\columnwidth]{AllFigures/Classification.pdf}
		\caption{Classification of related studies to be discussed in this survey.}
		\label{Fig::Classification}
	\end{center}
\end{figure} 

%The aforementioned surveys have no a full spectrum of reviews on access control, i.e., from data collection, data storage, and data usage, to blockchain (as a powerful tool for improving access control).
%, meanwhile considering CAAC, TBAC, GBAC, RAAC, and ReBAC.
%This survey aims to present and summarize the recent research work about access control technologies for edge computing, where CapBAC, ABE, PRE, DUC, GBAC, CAAC(basic, TBAC, RAAC, and ReBAC) are involved simultaneously.
%Therefore, it can prompt the development of access control technologies in edge computing under the intricacy of innovations in access control.








The rest of the paper is organized as follows. Section \ref{Sec::TraAccessControl} introduces typical access control models and blockchain technology with meaningful insights.
Section \ref{Sec::RAoAC} describes background knowledge about edge computing, and then presents our requirements analysis on access control in edge computing. 
Sections \ref{Sec::ACInDataCollection}\&\ref{Sec: ACInDataStorage}\&\ref{Sec::ACInDataUsage} respectively introduce the recent access control solutions according to the requirements. 
Further, Section \ref{Sec::Discussions} envisages some potential research directions to foster research efforts. 
Section \ref{Sec::SumAndCon} concludes this paper.  




==> Tex/SummaryAndConclusion.tex <==
\section{Conclusion}
\label{Sec::SumAndCon}
% This paper has effectively reviewed access control models for edge computing, which are crucial for low-latency, IoT-enabled applications like smart homes and autonomous vehicles.
% The paper identifies the unique challenges posed by edge computing environments, including limited resources at the edge, the need for low-latency processing, the dynamic nature of IoT device interactions, and the decentralized architecture.
% To conquer these challenges, the paper thoroughly classifies and evaluates various access control models, focusing on their effectiveness and efficiency in edge computing.
% The detailed classification encompasses the common data lifecycles—data collection, storage, and usage—highlighting how different models address the distinct challenges at each stage. Moreover, the paper systematically shows the role of blockchain technology as a potential solution to enhance the security and integrity of access control systems in edge environments. Blockchain's decentralized nature and immutability offer promising benefits to overcome some of the inherent vulnerabilities of traditional access control mechanisms, particularly in a distributed setting. 
% Through systematically exploring existing models and their adaptations to edge computing, the paper informs readers of the current state of access control techniques and underscores the need for continued innovation in this area. 



This paper has examined access control models applicable to edge computing, highlighting their critical role in enabling low-latency, IoT-driven applications like smart homes and autonomous vehicles. Systematically classifying these models and evaluating their effectiveness across different data lifecycles could assist readers in understanding access control technologies in edge computing, where the unique challenges include limited resources, the need for low-latency processing, dynamic interactions, and decentralized architectures.
Furthermore, the paper has effectively illustrated the potential of blockchain technology as a robust solution to enhance security and integrity within access control systems. The decentralized and immutable characteristics of blockchain are particularly beneficial in reinforcing the security measures necessary in distributed edge computing settings, where traditional access control mechanisms often fall short.
Through thoroughly exploring existing access control models and their adaptations to the unique demands of edge computing, the paper not only presents its readers with the state-of-the-art but also emphasizes the ongoing necessity for innovation. To match the fast-evolving IoT and edge computing landscape, we should create more adaptive, efficient, and secure access control solutions. Continued research is essential to fully leverage edge computing while maintaining data security.

%It calls for the development of more adaptive, efficient, and secure access control solutions that can keep pace with the rapidly evolving landscape of IoT applications and edge computing technology. This ongoing research and development will be crucial for harnessing the full potential of edge computing in various sectors, ensuring that data security keeps pace with technological advancements.

% In conclusion, while the paper presents a thorough exploration of current technologies and methodologies, it also underscores the ongoing need for research aimed at developing more scalable, efficient, and context-aware access control frameworks. These frameworks must not only address the inherent limitations and challenges of edge computing but also harness the potential of emerging technologies to foster a secure and resilient digital infrastructure. This is crucial for supporting the burgeoning growth of IoT applications and the increasing reliance on edge computing paradigms across various sectors.


% This paper has successfully surveyed the landscape of access control models applicable to edge computing, a vital domain characterized by its proximity to data sources and low latency operations, essential for IoT-enabled applications such as smart homes and autonomous vehicles. The study meticulously classifies and evaluates various access control models, considering their effectiveness and efficiency in the unique environment of edge computing, which often includes resource constraints and stringent security demands.


% The analysis reveals that while current models provide foundational security functionalities, evolving IoT applications and the increasing complexity of edge networks require novel solutions that can dynamically adapt to changing security landscapes and regulatory requirements without compromising performance.

% In conclusion, while the paper provides a comprehensive review of existing technologies, it also sets the stage for future research, highlighting the ongoing need for development of more robust, adaptable, and inherently secure access control solutions tailored for the rapidly growing and evolving field of edge computing. The continued exploration of blockchain and other emerging technologies could be key to achieving these advancements.


% Edge computing has many characteristics, e.g., low latency and resource constraints, which are challenging traditional access control solutions. The novel access control technologies are developing with the development of edge computing. From data collection, storage, and usage, to blockchain, we comprehensively analyzed the access control requirements according to the architecture of edge computing and reviewed recent research studies for corresponding access control. To motivate the development of access control technology in edge computing, we envisioned research directions for high-hybrid, intelligent access control, etc.

